On the Quantum Invariant for the Brieskorn Homology Spheres

We study an exact asymptotic behavior of the Witten-Reshetikhin-Turaev invariant for the Brieskorn homology spheres $\Sigma(p_1,p_2,p_3)$ by use of properties of the modular form following a method proposed by Lawrence and Zagier. Key observation is that the invariant coincides with a limiting value of the Eichler integral of the modular form with weight 3/2. We show that the Casson invariant is related to the number of the Eichler integrals which do not vanish in a limit $\tau\to N \in \mathbb{Z}$. Correspondingly there is a one-to-one correspondence between the non-vanishing Eichler integrals and the irreducible representation of the fundamental group, and the Chern-Simons invariant is given from the Eichler integral in this limit. It is also shown that the Ohtsuki invariant follows from a nearly modular property of the Eichler integral, and we give an explicit form in terms of the L-function.

==> pst-3dplot.tex <==
%%
%% This is file `pst-3dplot.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pst-3dplot.tex'
%%
%% Herbert Voss <voss@perce.de>
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-3dplot' is a PSTricks package to draw 3d curves and graphical objects
%%
\def\fileversion{1.30}
\def\filedate{2004/01/18}
\message{`PST-3dplot' v\fileversion, \filedate\space (Herbert Voss)}
\csname PSTThreeDplotLoaded\endcsname
\let\PSTThreeDplotLoaded\endinput
% Requires PSTricks, pst-node, pst-plot, multido packages
%\usepackage{pstcol}
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTnodesLoaded\endinput\else\input pst-node.tex\fi
\ifx\PSTplotLoaded\endinput\else\input pst-plot.tex\fi% plotpoints
\ifx\PSTNewThreeDLoaded\endinput\else\input pst-vue3d.tex\fi
\ifx\PSTMultidoLoaded\endinput\else\input multido.tex\fi
%
% DPC interface to the `keyval' package (until keyval based version of PSTricks)
\input pst-key
%
\edef\PstAtCode{\the\catcode`\@} \catcode`\@=11\relax
\SpecialCoor
%
%%%%%%%%%%%%%%%%%% Macrolist %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% \def\pstThreeDPut
% \def\pstThreeDLine
% \def\pstThreeDDot
% \def\pstThreeDNode
% \def\pstUThreeDPut
% \def\pstThreeDSquare
% \def\pstThreeDBox
% \def\pstThreeDSphere
% \def\pstThreeDEllipse
% \def\pstThreeDPlotFunc
% \def\psplotThreeD
% \def\parametricplotThreeD
% \def\psThreeDPlot
% \def\pstThreeDCoor
% \def\fileplotThreeD
% \def\dataplotThreeD
% \def\listplotThreeD
%
%
\newdimen\pst@dimf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ---------------- the if's -----------------
%
\newif\ifPst@drawing%			draw the coordinates?
\define@key{psset}{drawing}[true]{%
	\@nameuse{Pst@drawing#1}%
}
\newif\ifPst@drawCoor%		draw the coordinates of a dot?
\define@key{psset}{drawCoor}[false]{%
	\@nameuse{Pst@drawCoor#1}%
}
\newif\ifPst@hiddenLine%	emulate hidden line surface?
\define@key{psset}{hiddenLine}[false]{%
	\@nameuse{Pst@hiddenLine#1}%
}
\newif\ifPst@SphericalCoor% 	(r,phi,theta)
\define@key{psset}{SphericalCoor}[true]{\@nameuse{Pst@SphericalCoor#1}}
\setkeys{psset}{SphericalCoor=false}
%
% ------- the global definitions for the pspicture frame ------
%
\define@key{psset}{xMin}{\edef\psk@ThreeDplot@xMin{#1}}
\define@key{psset}{xMax}{\edef\psk@ThreeDplot@xMax{#1}}
\define@key{psset}{yMin}{\edef\psk@ThreeDplot@yMin{#1}}
\define@key{psset}{yMax}{\edef\psk@ThreeDplot@yMax{#1}}
\define@key{psset}{zMin}{\edef\psk@ThreeDplot@zMin{#1}}
\define@key{psset}{zMax}{\edef\psk@ThreeDplot@zMax{#1}}
\define@key{psset}{xThreeDunit}{\edef\psk@ThreeDplot@xThreeDunit{#1}}
\define@key{psset}{yThreeDunit}{\edef\psk@ThreeDplot@yThreeDunit{#1}}
\define@key{psset}{zThreeDunit}{\edef\psk@ThreeDplot@zThreeDunit{#1}}
%
% -------------- the angles and the plotpoints -------------
%
\define@key{psset}{Alpha}{%			Horizontal turn
	\edef\psk@ThreeDplot@Alpha{#1}%
}
\define@key{psset}{Beta}{%			Vertical turn
	\edef\psk@ThreeDplot@Beta{#1}%
}
\define@key{psset}{drawStyle}{%			how to draw 3D functions
	\edef\psk@ThreeDplot@drawStyle{#1}%
}
\def\drawStyle@xLines{xLines}
\def\drawStyle@yLines{yLines}
\def\drawStyle@xyLines{xyLines}
\def\drawStyle@yxLines{yxLines}
%
\define@key{psset}{xPlotpoints}{%		points in x direction
	\edef\psk@ThreeDplot@xPlotpoints{#1}%
}
\define@key{psset}{yPlotpoints}{%		points in y direction
	\edef\psk@ThreeDplot@yPlotpoints{#1}%
}
\define@key{psset}{beginAngle}{%		for ellipse/circle arc
	\edef\psk@ThreeDplot@beginAngle{#1}%
}
\define@key{psset}{endAngle}{%			for ellipse/circle arc
	\edef\psk@ThreeDplot@endAngle{#1}%
}
\define@key{psset}{linejoin}{%		how lines come together 0,1,2
	\edef\psk@ThreeDplot@linejoin{#1}%
}
\define@key{psset}{plane}{%			xy,xz,yz
	\edef\psk@ThreeDplot@plane{#1}%
}
\define@key{psset}{origin}{%			combination of (lr)(tBb)
	\edef\psk@ThreeDplot@origin{#1}%
}
\def\ThreeDplot@planeXY{xy}
\def\ThreeDplot@planeXZ{xz}
\def\ThreeDplot@planeYZ{yz}
%
% -------------- the length and node definitions -------------
%
\define@key{psset}{XO}{%			the X-offset
	\edef\psk@ThreeDplot@XO{#1}%
}
\define@key{psset}{YO}{%			the y-offset
	\edef\psk@ThreeDplot@YO{#1}%
}
\define@key{psset}{angleStep}{%		for circles
	\edef\psk@ThreeDplot@angleStep{#1}%
}
\define@key{psset}{posStart}{%		where the arrows start
	\edef\psk@ThreeDplot@posStart{#1}%
}
\define@key{psset}{length}{%		the length of the before|outlines
	\edef\psk@ThreeDplot@length{#1}%
}
\define@key{psset}{arrowOffset}{%	offset for \arrowLine
	\edef\psk@ThreeDplot@arrowOffset{#1}%
}
\define@key{psset}{visibleLineStyle}{%	offset for \arrowLine
	\edef\psk@ThreeDplot@visibleLineStyle{#1}%
}
\define@key{psset}{invisibleLineStyle}{%	offset for \arrowLine
	\edef\psk@ThreeDplot@invisibleLineStyle{#1}%
}
%
\define@key{psset}{nameX}{%		start of the object arrow
	\edef\psk@ThreeDplot@nameX{#1}%
}
\define@key{psset}{spotX}{%		where to draw the label
	\edef\psk@ThreeDplot@spotX{#1}%
}
\define@key{psset}{nameY}{%
	\edef\psk@ThreeDplot@nameY{#1}%
}
\define@key{psset}{spotY}{%
	\edef\psk@ThreeDplot@spotY{#1}%
}
\define@key{psset}{nameZ}{%
	\edef\psk@ThreeDplot@nameZ{#1}%
}
\define@key{psset}{spotZ}{%
	\edef\psk@ThreeDplot@spotZ{#1}%
}
%
\def\psds@none{\pst@gdot{}}% define none for the dotstyle
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                              %
%                        B A S I C S	                       %
%                                                              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\pstheader{pst-3dplot.pro}
\def\pst@3ddict{tx@3DPlotDict begin }
\def\tx@saveCoor{\pst@3ddict saveCoor end }
\def\tx@ConvertTo2D{\pst@3ddict ConvertTo2D end }
\def\tx@SphericalCoor{\pst@3ddict SphericalCoor end }
\def\tx@ConvertToCartesian{\pst@3ddict ConvertToCartesian end }
%
\def\setDefaults{%
    \setkeys{psset}{%
	drawing=true,hiddenLine=false,%
	xMin=-1,xMax=4,yMin=-1,yMax=4,zMin=-1,zMax=4,%
	xThreeDunit=1,yThreeDunit=1,zThreeDunit=1,%
	Alpha=45,Beta=30,%
	drawStyle=xLines,%
	xPlotpoints=25,yPlotpoints=25,%
	beginAngle=0,endAngle=360,%
	linejoin=1,%
	XO=0,YO=0,%
	angleStep=1,%
	posStart=0,length=2,%
	arrowOffset=0,%
	visibleLineStyle=solid,%
	invisibleLineStyle=dashed,%
	nameX=x,spotX=180,%
	nameY=y,spotY=0,%
	nameZ=z,spotZ=90,%
	plane=xy,origin=c,
	SphericalCoor=false%
    }%
}
\setDefaults
%
% (#1) -> #1 #2 #3
\def\getThreeDCoor#1#2{\pst@getThreeDcoor(#1)\let#2\pst@coorIIID}
\def\pst@getThreeDcoor(#1,#2,#3){%
	\edef\pst@coorIIID{#1\space #2\space #3\space}
}
\def\pst@addThreeDVec(#1)(#2)#3#4#5{%
	\pst@calcThreeDVec(#1)(#2)%
	\let#3\pst@getValueX%
	\let#4\pst@getValueY%
	\let#5\pst@getValueZ%
}
\def\pst@subThreeDVec(#1)(#2,#3,#4)#5#6#7{%
	\pst@calcThreeDVec(#1)(-#2,-#3,-#4)%
	\let#5\pst@getValueX%
	\let#6\pst@getValueY%
	\let#7\pst@getValueZ%
}
\def\pst@calcThreeDVec(#1,#2,#3)(#4,#5,#6){%
  \begingroup
    \pst@dima=#1 pt%
    \pst@dimb=#2 pt%
    \pst@dimc=#3 pt%
	\pst@dimf=#4 pt%
	\pst@dimg=#5 pt%
	\pst@dimh=#6 pt%
	\advance\pst@dima by \pst@dimf%
	\advance\pst@dimb by \pst@dimg%
	\advance\pst@dimc by \pst@dimh%
	\xdef\pst@getValueX{\pst@number\pst@dima}%
	\xdef\pst@getValueY{\pst@number\pst@dimb}%
	\xdef\pst@getValueZ{\pst@number\pst@dimc}%
  \endgroup
}%
%
% the ThreeD coordinate system
%
\def\pstThreeDCoor{\@ifnextchar[{\pst@ThreeDCoor}{\pst@ThreeDCoor[]}}
\def\pst@ThreeDCoor[#1]{{%
	\pst@killglue
	\setkeys{psset}{linewidth=0.5pt,linecolor=red,arrows=->,dotstyle=|}
	\setkeys{psset}{#1}
	\pstThreeDNode(\psk@ThreeDplot@xMin,0,0){xMin}
	\pstThreeDNode(\psk@ThreeDplot@xMax,0,0){xMax}
	\pstThreeDNode(0,\psk@ThreeDplot@yMin,0){yMin}
	\pstThreeDNode(0,\psk@ThreeDplot@yMax,0){yMax}
	\pstThreeDNode(0,0,\psk@ThreeDplot@zMin){zMin}
	\pstThreeDNode(0,0,\psk@ThreeDplot@zMax){zMax}
	\ifPst@drawing
	    % ThreeDplot axes
	    \psline(xMin)(xMax)
	    \psline(yMin)(yMax)
	    \psline(zMin)(zMax)
	    \uput[\psk@ThreeDplot@spotX](xMax){$\mathbf{\psk@ThreeDplot@nameX}$}
	    \uput[\psk@ThreeDplot@spotY](yMax){$\mathbf{\psk@ThreeDplot@nameY}$}
	    \uput[\psk@ThreeDplot@spotZ](zMax){$\mathbf{\psk@ThreeDplot@nameZ}$}
	\fi% ifdrawing
}}
%
% put anything at (#2,#3,#4)
%
\def\pstThreeDPut{\@ifnextchar[{\pst@ThreeDPut}{\pst@ThreeDPut[]}}
\def\pst@ThreeDPut[#1](#2,#3,#4)#5{{%
	\pst@killglue%
	\setkeys{psset}{#1}
	\pstThreeDNode(#2,#3,#4){temp@pstNode}%
%	\def\@tempa{c}
%	\ifx\pst@ThreeDplot@origin\@tempa%
%	    \rput(temp@pstNode){#5}%
%	\else%
	    \rput[\psk@ThreeDplot@origin](temp@pstNode){#5}%
%	\fi%
}}
%
% draws a 3d line
%
\def\cartesianIIID@coor#1,#2,#3,#4\@nil{\edef\pst@coor{#1 #2 #3 }}
\def\NormalIIIDCoor{%
    \def\pst@@getcoor##1{\pst@expandafter\cartesianIIID@coor{##1},\relax,\@nil}%
    \def\pst@@getangle##1{%
        \pst@checknum{##1}\pst@angle
        \edef\pst@angle{\pst@angle \pst@angleunit}%
    }%
    \def\psput@##1{\pst@@getcoor{##1}\leavevmode\psput@cartesian}%
}
\def\pstThreeDLine{\NormalIIIDCoor\pst@object{lineIIID}}
\def\lineIIID@i{%
    \pst@getarrows{%
        \begin@OpenObj
        \pst@getcoors[\lineIIID@ii%
    }%
}
\def\lineIIID@ii{%
    \addto@pscode{%
		\pst@3ddict
		/Alpha \psk@ThreeDplot@Alpha\space def %
		/Beta \psk@ThreeDplot@Beta\space def %
		/SphericalCoor {\ifPst@SphericalCoor true \else false \fi} def %
		/xUnit { \pst@number\psxunit\space mul } def
		/yUnit { \pst@number\psyunit\space mul } def
		convertStackTo2D
		end
		\pst@cp \psline@iii \tx@Line%
	}%
    \end@OpenObj%
	\SpecialCoor%
}
%
% set a 3d dot
%
\def\pstThreeDDot{\@ifnextchar[{\pst@ThreeDDot}{\pst@ThreeDDot[]}}
\def\pst@ThreeDDot[#1](#2,#3,#4){{%
%	\pst@killglue
	\setkeys{psset}{linestyle=dashed,linewidth=0.5pt}% default
	\setkeys{psset}{#1}
	\pstThreeDNode[#1](#2,#3,#4){A}
	\ifx\psk@dotstyle\@none\else\psdots(A)\fi
	\ifPst@drawCoor
		\pnode(!%
			\pst@3ddict
			/Alpha \psk@ThreeDplot@Alpha\space def
			/Beta \psk@ThreeDplot@Beta\space def
			\ifPst@SphericalCoor
				#2\space #3\space #4\space
				ConvertToCartesian /z 0 def
			\else
				/x #2 def /y #3 def /z 0 def
			\fi
		ConvertTo2D x2D y2D end ){B}
		\psline(A)(B)
		\pnode(!%   y=0, z=0
			\pst@3ddict
			\ifPst@SphericalCoor
				#2\space #3\space #4\space
				ConvertToCartesian /y 0 def /z 0 def
			\else
				/x #2 def /y 0 def /z 0 def
			\fi
		ConvertTo2D x2D y2D end ){A}%
		\psline(B)(A)%
		\pnode(!%   x=0, z=0
			\pst@3ddict
			\ifPst@SphericalCoor
				#2\space #3\space #4\space
				ConvertToCartesian /x 0 def /z 0 def
			\else
				/x 0 def /y #3 def /z 0 def
			\fi
		ConvertTo2D x2D y2D end ){A}%
		\psline(B)(A)
	\fi
}}
%
% transform the 3d coordinates of the node (#1,#2,#3)
% into a 2d node with the name #4
%
\def\pstThreeDNode{\@ifnextchar[{\pst@ThreeDNode}{\pst@ThreeDNode[]}}
\def\pst@ThreeDNode[#1](#2,#3,#4)#5{{%
	\psset{#1}
	\pnode(!%
		\pst@3ddict
		/Alpha \psk@ThreeDplot@Alpha\space def
		/Beta \psk@ThreeDplot@Beta\space def
		\ifPst@SphericalCoor
			#2\space #3\space #4\space
			ConvertToCartesian
		\else
			/x #2 def /y #3 def /z #4 def
		\fi
		ConvertTo2D x2D y2D end){#5}%
}}
%
% a 3d uput[](){}
%
\def\pstUThreeDPut{\@ifnextchar[{\pst@UThreeDPut}{\pst@UThreeDPut[]}}
\def\pst@UThreeDPut[#1](#2,#3,#4)#5{{%
	\uput[#1](!%
		\pst@3ddict
		/Alpha \psk@ThreeDplot@Alpha\space def
		/Beta \psk@ThreeDplot@Beta\space def
		\ifPst@SphericalCoor
			#2\space #3\space #4\space
			ConvertToCartesian
		\else
			/x #2 def /y #3 def /z #4 def
		\fi
		ConvertTo2D x2D y2D end){#5}
}}
%
% Trangle [options](Point1)(Point2)(Point3)
%
\def\pstThreeDTriangle{%
	\@ifnextchar[%
		{\do@ThreeDTriangle}%
		{\do@ThreeDTriangle[]}%
}
\def\do@ThreeDTriangle[#1](#2)(#3)(#4){{%
	\ifx#1\empty\else\setkeys{psset}{#1}\fi%
	\ifPst@drawCoor
		\pstThreeDDot[drawCoor=true](#2)%
		\pstThreeDDot[drawCoor=true](#3)%
		\pstThreeDDot[drawCoor=true](#4)%
	\fi
	\pstThreeDNode(#2){A}
	\pstThreeDNode(#3){B}
	\pstThreeDNode(#4){C}
	\ifx\psk@fillstyle\@none
	\else
		\pscustom{%
			\code{\psk@ThreeDplot@linejoin\space setlinejoin}%
	\fi%
		\psline[#1](A)(B)(C)(A)
	\ifx\psk@fillstyle\@none\else}\fi%
}}
%
% draws a threeD square as a polygon
%
% [#1] options
% (#2) starting vector ax,ay,az
% (#3) first direction vector ux,uy,uz
% (#4) second direction vector wx,wy,wz
%
\def\pstThreeDSquare{\pst@object{squareIIID}}
\def\squareIIID@i{\squareIIID@ii}
\def\squareIIID@ii(#1)(#2)(#3){%
	\ifPst@drawCoor%
		{%
		\psset{linestyle=dashed,linewidth=0.5pt}%
		\pstThreeDDot(#1)%
		\pst@addThreeDVec(#1)(#2)\pst@tempa\pst@tempb\pst@tempc%
		\pstThreeDDot(\pst@tempa,\pst@tempb,\pst@tempc)%
		\pst@addThreeDVec(#1)(#3)\pst@tempa\pst@tempb\pst@tempc
		\pstThreeDDot(\pst@tempa,\pst@tempb,\pst@tempc)%
		\pst@addThreeDVec(\pst@tempa,\pst@tempb,\pst@tempc)%
			(#2)\pst@tempa\pst@tempb\pst@tempc%
		\pstThreeDDot(\pst@tempa,\pst@tempb,\pst@tempc)%
		}%
	\fi%
	\getThreeDCoor{#1}\pst@tempa%
	\getThreeDCoor{#2}\pst@tempb%
	\getThreeDCoor{#3}\pst@tempc%
	\begin@OpenObj
		\addto@pscode{%
			/P1 {\pst@tempa } def % x y z or Radius longitude lattitude
			/P2 {\pst@tempb } def %
			/P3 {\pst@tempc } def %
			/Alpha \psk@ThreeDplot@Alpha\space def %
			/Beta \psk@ThreeDplot@Beta\space def %
			/SphericalCoor \ifPst@SphericalCoor true \else false \fi def %
			/xUnit { \pst@number\psxunit\space mul } def
			/yUnit { \pst@number\psyunit\space mul } def
			\pst@3ddict
			P1 saveCoor
			SphericalCoor {ConvertToCartesian} if
			ConvertTo2D
			/x0 x2D xUnit def /y0 y2D yUnit def
			P2 saveCoor
			SphericalCoor {ConvertToCartesian} if
			ConvertTo2D
			/x1 x2D xUnit x0 add def /y1 y2D yUnit y0 add def
			P3 saveCoor
			SphericalCoor {ConvertToCartesian} if
			ConvertTo2D
			/x2 x2D xUnit x1 add def /y2 y2D yUnit y1 add def
			P2 saveCoor
			SphericalCoor {ConvertToCartesian} if
			ConvertTo2D
			/x3 x2D xUnit neg x2 add def /y3 y2D yUnit neg y2 add def
			[ x0 y0 x1 y1 x2 y2 x3 y3 x0 y0
			\pst@cp \psline@iii \tx@Line
			end
		}%
    \end@OpenObj%
}

%
% draws a threeD Box
% [#1] options
% (#2) first direction vector ux,uy,uz
% (#3) second direction vector vx,vy,vz
% (#4) third direction vector wx,wy,wz
%
\def\pstThreeDBox{\@ifnextchar[{\doThreeDBox}{\doThreeDBox[]}}
\def\doThreeDBox[#1](#2)(#3)(#4)(#5){{
	\psset{linestyle=\psk@ThreeDplot@invisibleLineStyle}
	\psset{#1}
	%
%	\psset{linestyle=dashed}
%	\psset{linestyle=\psk@ThreeDplot@invisibleLineStyle}
	\addto@par{linestyle=\psk@ThreeDplot@invisibleLineStyle}
	\pstThreeDSquare[#1](#2)(#4)(#5) % 	lower square
	\pstThreeDSquare(#2)(#3)(#4)% 	back square
	%
	\psset{linestyle=\psk@ThreeDplot@visibleLineStyle}
	\pst@addThreeDVec(#2)(#4)\pst@tempa\pst@tempb\pst@tempc
	\pstThreeDSquare(\pst@tempa,\pst@tempb,\pst@tempc)(#3)(#5)% left square
	\pst@addThreeDVec(#2)(#3)\pst@tempa\pst@tempb\pst@tempc
	\pstThreeDSquare(\pst@tempa,\pst@tempb,\pst@tempc)(#4)(#5)% top square
	\pst@addThreeDVec(#2)(#5)\pst@tempa\pst@tempb\pst@tempc
	\pstThreeDSquare(\pst@tempa,\pst@tempb,\pst@tempc)(#3)(#4)% front square
	%
}}
%
% Sphere
%
\def\pstThreeDSphere{\@ifnextchar[{\pst@ThreeDSphere}{\pst@ThreeDSphere[]}}
\def\pst@ThreeDSphere[#1](#2,#3,#4)#5{{%
	\psset{THETA=\psk@ThreeDplot@Beta,PHI=\psk@ThreeDplot@Beta,%
		Dobs=10,Decran=10}
	\psset{#1}
	\pstThreeDNode(#2,#3,#4){SphereCenter}
	\rput(SphereCenter){\SphereThreeD(0,0,0){#5}}
}}
%
% set a 3d ellipse/circle
%
% #1 options
% #2 center cx,cy,cz
% #3 radius ax,ay,az
% #4 radius bx,by,bz
%
\def\pstThreeDEllipse{\@ifnextchar[{\doThreeDEllipse}{\doThreeDEllipse[]}}
\def\doThreeDEllipse[#1](#2)(#3)(#4){{%
	\psset{plotstyle=curve,xPlotpoints=\psk@plotpoints}
	\psset{#1}
	\getThreeDCoor{#2}\pst@tempc%	 center
	\getThreeDCoor{#3}\pst@tempa%	 a
	\getThreeDCoor{#4}\pst@tempb%	 b
	\parametricplotThreeD(\psk@ThreeDplot@beginAngle,\psk@ThreeDplot@endAngle){%
		\pst@3ddict
		\pst@tempc\space
		\ifPst@SphericalCoor
			ConvertToCartesian x y z
		\fi
		\pst@tempa\space
		\ifPst@SphericalCoor
			ConvertToCartesian x y z
		\fi
		\pst@tempb\space
		\ifPst@SphericalCoor
			ConvertToCartesian x y z
		\fi
		9 -1 roll t cos 8 -1 roll neg mul add t sin 5 -1 roll mul add
		7 -1 roll t cos 7 -1 roll neg mul add t sin 5 -1 roll mul add
		5 -1 roll t cos 6 -1 roll neg mul add t sin 5 -1 roll mul add
		end
	}
}}
%
\def\pstThreeDCircle{\pstThreeDEllipse}
\def\pstThreeDPlotFunc{\psplotThreeD}%	only for compatibility
%
\def\pstRotPoint{\@ifnextchar[{\pstRotPointi}{\pstRotPointi[]}}
\def\pstRotPointi[#1](#2,#3,#4)(#5,#6,#7)#8{{%
	\setkeys{psset}{#1}
	\def\pst@ThreeDplot@ThetaX{#5}	% rotating angle
	\def\pst@ThreeDplot@ThetaY{#6}	% rotating angle
	\def\pst@ThreeDplot@ThetaZ{#7}	% rotating angle
	\pnode(!%
		\pst@3ddict
		/Alpha \psk@ThreeDplot@Alpha\space def
		/Beta \psk@ThreeDplot@Beta\space def
		\ifPst@SphericalCoor
			#2\space #3\space #4\space
			ConvertToCartesian
		\else
			/x #2 def /y #3 def /z #4 def
		\fi
% rotating on the z-Axes
		/Theta \pst@ThreeDplot@ThetaZ\space def
		/x0 x Theta cos mul y Theta sin mul sub def
		/y x Theta sin mul y Theta cos mul add def
		/x x0 def
% rotating on the y-Axes
		/Theta \pst@ThreeDplot@ThetaY\space def
		/x0 x Theta cos mul z Theta sin mul add def
		/z x neg Theta sin mul z Theta cos mul add def
		/x x0 def
% rotating on the x-Axes
		/Theta \pst@ThreeDplot@ThetaX\space def
		/y0 y Theta cos mul z Theta sin mul sub def
		/z y Theta sin mul z Theta cos mul add def
		/y y0 def
%
		ConvertTo2D x2D y2D end){#8}
}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\psplotinit#1{\xdef\psplot@init{#1 }}
\def\psplot@init{}
%
\def\psplotThreeD{\@ifnextchar[{\ps@plotThreeD}{\ps@plotThreeD[]}}
\def\ps@plotThreeD[#1](#2,#3)(#4,#5)#6{%
    \setkeys{psset}{hiddenLine=false,drawStyle=xLines}% default
    \setkeys{psset}{#1}
    \ifx\psk@ThreeDplot@drawStyle\drawStyle@xyLines
	\doPlotThreeD@xLines(#2,#3)(#4,#5){#6}
	\doPlotThreeD@yLines(#2,#3)(#4,#5){#6}
    \else
	\ifx\psk@ThreeDplot@drawStyle\drawStyle@yxLines
	    \doPlotThreeD@yLines(#2,#3)(#4,#5){#6}
	    \doPlotThreeD@xLines(#2,#3)(#4,#5){#6}
	\else
	    \ifx\psk@ThreeDplot@drawStyle\drawStyle@xLines
		\doPlotThreeD@xLines(#2,#3)(#4,#5){#6}
	    \fi
	    \ifx\psk@ThreeDplot@drawStyle\drawStyle@yLines
		\doPlotThreeD@yLines(#2,#3)(#4,#5){#6}
	    \fi
	\fi
    \fi
}
\def\doPlotThreeD@xLines{%
	\def\pst@par{}
	\pst@object{psplotThreeD@xLines}%
}
\def\doPlotThreeD@yLines{%
	\def\pst@par{}
	\pst@object{psplotThreeD@yLines}%
}
\def\psplotThreeD@xLines@i(#1,#2)(#3,#4)#5{%
    \pst@killglue
    \begingroup
	\use@par%
	\@pstfalse
	\@nameuse{beginplot@\psplotstyle}%
	\gdef\psplot@init{}%
	\@nameuse{testqp@\psplotstyle}%
	\if@pst%	lines and dots
	    \addto@pscode{%
		/Alpha \psk@ThreeDplot@Alpha\space def
		/Beta \psk@ThreeDplot@Beta\space def
		/xMin #1 def
		/x xMin def
		/x1 #2 def
		/y #3 def
		/y1 #4 def
		/dx x1 x sub \psk@ThreeDplot@xPlotpoints\space div def
		/dy y1 y sub \psk@ThreeDplot@yPlotpoints\space div def
		/func {#5} def
		/xyz {
		    x neg Alpha cos mul y Alpha sin mul add \pst@number\psxunit mul
		    x Alpha sin mul y Alpha cos mul add neg Beta sin mul
			func Beta cos mul add \pst@number\psyunit mul} def
	    }%
	    \psplotThreeD@xLines@ii
	\else%	curves
	    \endgroup
	    \multido{\n@Y=0+1}{\psk@ThreeDplot@yPlotpoints}{%
		\ifPst@hiddenLine\pscustom[fillcolor=white,fillstyle=solid]{\fi
		    \@nameuse{beginplot@\psplotstyle}%
			\addto@pscode{%
			    /Alpha \psk@ThreeDplot@Alpha\space def
			    /Beta \psk@ThreeDplot@Beta\space def
			    /xMin #1 def
			    /x xMin def
			    /x1 #2 def
			    /dx x1 x sub \psk@ThreeDplot@xPlotpoints\space div def
			    /dy #4\space #3\space sub \psk@ThreeDplot@yPlotpoints\space div def
			    /y #3\space \n@Y\space dy mul add def
			    /func {#5} def
			    /xyz {
				x neg Alpha cos mul y Alpha sin mul add \pst@number\psxunit mul
				x Alpha sin mul y Alpha cos mul add neg Beta sin mul
				    func Beta cos mul add \pst@number\psyunit mul} def
			}%
		    \psplotThreeD@xLines@iii%
		\ifPst@hiddenLine }\fi%
	    }%
	\fi
    \endgroup
    \ignorespaces%
}
\def\psplotThreeD@xLines@ii{%
    \addto@pscode{%
	xyz \@nameuse{beginqp@\psplotstyle}
	\psk@ThreeDplot@yPlotpoints\space 1 add {
	    /x xMin def
	    xyz moveto
	    \psk@ThreeDplot@xPlotpoints\space 1 add {
		xyz \@nameuse{doqp@\psplotstyle}
		/x x dx add def
	    } repeat
	    /y y dy add def
	} repeat
	/x x1 def
	/y y1 def
	xyz \@nameuse{doqp@\psplotstyle}
    }%
    \@nameuse{endqp@\psplotstyle}%
}
\def\psplotThreeD@xLines@iii{%    curves
    \addto@pscode{%
	    /x xMin def
	    mark
	    /n 2 def
		\psk@ThreeDplot@xPlotpoints {
	    	    xyz
    		    n 2 roll
    		    /n n 2 add def
    		    /x x dx add def
    		} repeat
        /x x1 def
        xyz
        n 2 roll
    }%
    \@nameuse{endplot@\psplotstyle}%
}
%
\def\psplotThreeD@yLines@i(#1,#2)(#3,#4)#5{%
    \pst@killglue
    \begingroup
	\use@par%
	\@pstfalse
	\@nameuse{beginplot@\psplotstyle}%
	\gdef\psplot@init{}%
	\@nameuse{testqp@\psplotstyle}%
	\if@pst%	lines and dots
	    \addto@pscode{%
		/Alpha \psk@ThreeDplot@Alpha\space def
		/Beta \psk@ThreeDplot@Beta\space def
    		/x #1 def
		/x1 #2 def
		/yMin #3 def
		/y yMin def
		/y1 #4 def
		/dx x1 x sub \psk@ThreeDplot@xPlotpoints\space div def
		/dy y1 y sub \psk@ThreeDplot@yPlotpoints\space div def
		/func {#5} def
		/xyz {
		    x neg Alpha cos mul y Alpha sin mul add \pst@number\psxunit mul
		    x Alpha sin mul y Alpha cos mul add neg Beta sin mul
			func Beta cos mul add \pst@number\psyunit mul} def
	    }%
	    \psplotThreeD@yLines@ii
	\else%	curves
	    \endgroup
	    \multido{\n@X=0+1}{\psk@ThreeDplot@xPlotpoints}{%
		\ifPst@hiddenLine\pscustom[fillcolor=white,fillstyle=solid]{\fi
		    \@nameuse{beginplot@\psplotstyle}%
			\addto@pscode{%
			    /Alpha \psk@ThreeDplot@Alpha\space def
			    /Beta \psk@ThreeDplot@Beta\space def
			    /yMin #3 def
			    /y yMin def
			    /y1 #4 def
			    /dy y1 y sub \psk@ThreeDplot@yPlotpoints\space div def
			    /dx #2\space #1\space sub \psk@ThreeDplot@xPlotpoints\space div def
			    /x #1\space \n@X\space dx mul add def
			    /func {#5} def
			    /xyz {
				x neg Alpha cos mul y Alpha sin mul add \pst@number\psxunit mul
				x Alpha sin mul y Alpha cos mul add neg Beta sin mul
				    func Beta cos mul add \pst@number\psyunit mul} def
			}%
		    \psplotThreeD@yLines@iii%
		\ifPst@hiddenLine }\fi%
	    }%
	\fi
    \endgroup
    \ignorespaces%
}
\def\psplotThreeD@yLines@ii{%
    \addto@pscode{%
	xyz \@nameuse{beginqp@\psplotstyle}
	\psk@ThreeDplot@xPlotpoints\space 1 add {
	    /y yMin def
	    xyz moveto
	    \psk@ThreeDplot@yPlotpoints\space 1 add {
		xyz \@nameuse{doqp@\psplotstyle}
		/y y dy add def
	    } repeat
	    /x x dx add def
	} repeat
	/x x1 def
	/y y1 def
	xyz \@nameuse{doqp@\psplotstyle}
    }%
    \@nameuse{endqp@\psplotstyle}%
}
\def\psplotThreeD@yLines@iii{%    curves
    \addto@pscode{%
	    /y yMin def
	    mark
	    /n 2 def
		\psk@ThreeDplot@yPlotpoints {
	    	    xyz
    		    n 2 roll
    		    /n n 2 add def
    		    /y y dy add def
    		} repeat
        /y y1 def
        xyz
        n 2 roll
    }%
    \@nameuse{endplot@\psplotstyle}%
}
%
% parametricplot ----------------------------------------------------------------
%
\def\parametricplotThreeD{%
	\@ifnextchar[{\doParametricPlotThreeD}{\doParametricPlotThreeD[]}%
}
\def\doParametricPlotThreeD[#1]{%
	\setkeys{psset}{#1}%
	\def\pst@par{}%
	\pst@object{psParamPlotThreeD}%
}
\def\psParamPlotThreeD@i(#1){%
	\@ifnextchar({\psParamPlotThreeD@ii(#1)}{\psParamPlotThreeD@ii(#1)(0,0)}%
}
\def\psParamPlotThreeD@ii(#1,#2)(#3,#4)#5 {%
    \pst@killglue
    \begingroup
	\use@par%
	\@pstfalse
	\@nameuse{beginplot@\psplotstyle}%
	\gdef\parametricII@init{}%
	\@nameuse{testqp@\psplotstyle}%
	\if@pst
	    \addto@pscode{%
	    	/Alpha \psk@ThreeDplot@Alpha\space def
	    	/Beta \psk@ThreeDplot@Beta\space def
		/tMin #1 def
		/t tMin def
		/t1 #2 def
		/u #3 def
		/u1 #4 def
		/dt t1 t sub \psk@ThreeDplot@xPlotpoints\space div def
		/du u1 u sub \psk@ThreeDplot@yPlotpoints\space div def
		/xyz {
		    #5
		    3 -1 roll               % y z x
		    \psk@ThreeDplot@xThreeDunit\space div
		    dup                     % y z x x
		    neg Alpha cos mul       % y z x (x)
		    4 -1 roll               % z x (x) y
		    \psk@ThreeDplot@yThreeDunit\space div
		    dup                     % z x (x) y y
		    5 1 roll                % y z x (x) y
		    Alpha sin mul add \pst@number\psxunit mul       % y z x (x2)
		    4 1 roll                % (x2) y z x
		    Alpha sin mul           % (x2) y z (x)
		    3 -1 roll               % (x2) z (x) y
		    Alpha cos mul add neg Beta sin mul % (x2) z (x)
		    exch                    % (x2) (x) z
		    \psk@ThreeDplot@zThreeDunit\space div
		    Beta cos mul add \pst@number\psyunit mul        % (x2) (y2)
		} def
	    }%
	    \psParamPlotThreeD@iii%
	\else
	    \endgroup
	    \ifx#3#4\psset{yPlotpoints=1}\fi% do we have two different parameters or #3=#4
		\multido{\n@Y=0+1}{\psk@ThreeDplot@yPlotpoints}{%
		\@nameuse{beginplot@\psplotstyle}%
		\addto@pscode{%
		    /Alpha \psk@ThreeDplot@Alpha\space def
		    /Beta \psk@ThreeDplot@Beta\space def
		    /tMin #1 def
		    /t tMin def
		    /t1 #2 def
		    /dt t1 t sub \psk@ThreeDplot@xPlotpoints\space div def
		    /du #4\space #3\space sub \psk@ThreeDplot@yPlotpoints\space div def
		    /u #3\space \n@Y\space du mul add def
		    /xyz {
			#5
			3 -1 roll               % y z x
			\psk@ThreeDplot@xThreeDunit\space div
			dup                     % y z x x
			neg Alpha cos mul       % y z x (x)
			4 -1 roll               % z x (x) y
			\psk@ThreeDplot@yThreeDunit\space div
			dup                     % z x (x) y y
			5 1 roll                % y z x (x) y
			Alpha sin mul add \pst@number\psxunit mul       % y z x (x2)
			4 1 roll                % (x2) y z x
			Alpha sin mul           % (x2) y z (x)
			3 -1 roll               % (x2) z (x) y
			Alpha cos mul add neg Beta sin mul % (x2) z (x)
			exch                    % (x2) (x) z
			\psk@ThreeDplot@zThreeDunit\space div
			Beta cos mul add \pst@number\psyunit mul        % (x2) (y2)
		    } def
		}%
		\psParamPlotThreeD@iv%
	    }%
	\fi
    \endgroup
    \ignorespaces%
}
\def\psParamPlotThreeD@iii{%
    \addto@pscode{%
	xyz \@nameuse{beginqp@\psplotstyle}
	\psk@ThreeDplot@yPlotpoints\space 1 add {
	    /t tMin def
	    xyz moveto
	    \psk@ThreeDplot@xPlotpoints\space 1 add {
		xyz \@nameuse{doqp@\psplotstyle}
		/t t dt add def
	    } repeat
	    /u u du add def
	} repeat
	/t u1 def
	/u u1 def
	xyz \@nameuse{doqp@\psplotstyle}
    }%
    \@nameuse{endqp@\psplotstyle}%
}
\def\psParamPlotThreeD@iv{%
	\addto@pscode{%
%	    /t tMin def
		mark
	    /n 2 def
		\psk@ThreeDplot@xPlotpoints {
			xyz
    		n 2 roll
    		/n n 2 add def
    		/t t dt add def
		} repeat
		/t t1 def
		xyz
		n 2 roll
    }%
	\@nameuse{endplot@\psplotstyle}%
}
%
% Plot 3D data
%
\def\fileplotThreeD{\def\pst@par{}\pst@object{fileplotThreeD}}
\def\fileplotThreeD@i#1{%
    \pst@killglue
    \begingroup
	\use@par
	\@pstfalse
	\@nameuse{testqp@\psplotstyle}%
	\if@pst
	    \dataplotThreeD@ii{\pst@readfile{#1}}%
	\else
	    \listplotThreeD@ii{\pst@altreadfile{#1}}%
	\fi
    \endgroup
    \ignorespaces%
}
%
% dataplot
%
\def\dataplotThreeD{\def\pst@par{}\pst@object{dataplotThreeD}}
\def\dataplotThreeD@i#1{%
  \pst@killglue
  \begingroup
    \use@par
    \@pstfalse
    \@nameuse{testqp@\psplotstyle}%
    \if@pst
      \dataplotThreeD@ii{\addto@pscode{#1}}%
    \else
      \listplot@ii{\addto@pscode{#1}}%
    \fi
  \endgroup
  \ignorespaces%
}
\def\dataplotThreeD@ii#1{%
  \@nameuse{beginplot@\psplotstyle}%
    \addto@pscode{%
      /Alpha \psk@ThreeDplot@Alpha\space def
      /Beta \psk@ThreeDplot@Beta\space def
      /Dx { /D { Dy } def } def
      /Dy { /D { Dz } def } def
      /Dz { 			% now we have x y z
	3 -1 roll		% y z x
        \psk@ThreeDplot@xThreeDunit\space div
	dup			% y z x x
	neg Alpha cos mul	% y z x (x)
	4 -1 roll		% z x (x) y
	\psk@ThreeDplot@yThreeDunit\space div
	dup			% z x (x) y y
	5 1 roll		% y z x (x) y
	Alpha sin mul add \pst@number\psxunit mul % y z x (x2)
	4 1 roll		% (x2) y z x
	Alpha sin mul		% (x2) y z (x)
	3 -1 roll		% (x2) z (x) y
	Alpha cos mul add neg Beta sin mul % (x2) z (x)
	exch			% (x2) (x) z
	\psk@ThreeDplot@zThreeDunit\space div
	Beta cos mul add \pst@number\psyunit mul % (x2) (y2)
	Do /D { Dx } def } def
      /D { /D { Dx } def } def
      /Do {
        \@nameuse{beginqp@\psplotstyle}%
        /Do { \@nameuse{doqp@\psplotstyle}} def
      } def}%
    #1%
    \addto@pscode{D}%
  \@nameuse{endqp@\psplotstyle}%
}
%
%
\pst@def{ScalePointsThreeD}<%
	counttomark dup dup cvi eq not { exch pop } if
	/m exch def /n m 3 div cvi def
	n { 				% now we have x y z
		3 -1 roll		% y z x
		\psk@ThreeDplot@xThreeDunit\space div
		dup			% y z x x
		neg Alpha cos mul	% y z x (x)
		4 -1 roll		% z x (x) y
		\psk@ThreeDplot@yThreeDunit\space div
		dup			% z x (x) y y
		5 1 roll		% y z x (x) y
		Alpha sin mul add \pst@number\psxunit mul	% y z x (x2)
		4 1 roll		% (x2) y z x
		Alpha sin mul		% (x2) y z (x)
		3 -1 roll		% (x2) z (x) y
		Alpha cos mul add neg Beta sin mul % (x2) z (x)
		exch			% (x2) (x) z
		\psk@ThreeDplot@zThreeDunit\space div
		Beta cos mul add \pst@number\psyunit mul 	% (x2) (y2)
		m 1 sub 1 roll m 1 sub 1 roll /m m 3 sub def } repeat>
%
% listplotThreeD
%
\def\listplotThreeD{\def\pst@par{}\pst@object{listplotThreeD}}
\def\listplotThreeD@i#1{\listplotThreeD@ii{\addto@pscode{#1}}}
\def\listplotThreeD@ii#1{%
	\@nameuse{beginplot@\psplotstyle}%
	\addto@pscode{%
		/Alpha \psk@ThreeDplot@Alpha\space def
		/Beta \psk@ThreeDplot@Beta\space def
		/D {} def mark %
	}%
	#1%
	\addto@pscode{\tx@ScalePointsThreeD}%
	\@nameuse{endplot@\psplotstyle}%
}
%
% adopted from pst-3d
%
\pst@def{TMSave}<%
  tx@Dict /TMatrix known not { /TMatrix { } def /RAngle { 0 } def } if
  /TMatrix [ TMatrix CM ] cvx def>
%
\pst@def{TMRestore}<%
  CP /TMatrix [ TMatrix setmatrix ] cvx def moveto>
%
\pst@def{TMChange}<%
  \tx@TMSave
  /cp [ currentpoint ] cvx def
  CM
  CP T \tx@STV
  CM matrix invertmatrix 
  matrix concatmatrix
  exch exec
  concat cp moveto>
%
\def\pstPlanePut{\@ifnextchar[{\pst@PlanePut}{\pst@PlanePut[]}}
\def\pst@PlanePut[#1](#2)#3{{%
	\pst@killglue%
	\setkeys{psset}{origin=lB}%
	\setkeys{psset}{#1}%
	\pstThreeDPut[#1](#2){\ps@Plane{#3}}%
}}
%
\def\ps@Plane{\pst@makebox{\psPlane@}}
\def\psPlane@{%
    \begingroup
	\leavevmode%
    	\hbox{%
%	    \kern\wd\pst@hbox%
	    \pst@Verb{%
		{ [ 1 0
		    /Alpha \psk@ThreeDplot@Alpha\space def
		    /Beta \psk@ThreeDplot@Beta\space def
		    /Delta Beta sin Alpha sin mul Alpha cos atan neg 90 add def 
		    /Gamma Beta sin Alpha cos mul neg Alpha sin atan def 
		    \ifx\psk@ThreeDplot@plane\ThreeDplot@planeXY
			270 Delta sub rotate
			/Rho 90 Gamma add Delta add def
		    \else%
			\ifx\psk@ThreeDplot@plane\ThreeDplot@planeXZ
		    	    270 Delta sub rotate
 			    /Rho 180 Delta add def
			\else%
		    	    Gamma rotate
			    /Rho 90 Gamma sub def
			\fi%
		    \fi%
		    Rho cos Rho sin 0 0 ] concat} \tx@TMChange%
	    }%
	    \box\pst@hbox%
	    \pst@Verb{\tx@TMRestore}%
%	    \kern\ht\pst@hbox%
	}%
    \endgroup%
}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Utility stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% posStart=Starting point
% length=  Arrow length.
\def\Arrows{\@ifnextchar[{\pst@Arrows}{\pst@Arrows[]}}
\def\pst@Arrows[#1](#2)(#3){{%
	\setkeys{psset}{#1}%
	\pst@getcoor{#2}\pst@tempa
	\pst@getcoor{#3}\pst@tempb
	\pnode(!%
		/StartArrow \psk@ThreeDplot@posStart\space def
		/LengthArrow \psk@ThreeDplot@length\space def
		\pst@tempa /YA exch \pst@number\psyunit div def
		/XA exch \pst@number\psxunit div def
		\pst@tempb /YB exch \pst@number\psyunit div def
		/XB exch \pst@number\psxunit div def
		/denominateur XB XA sub def
		/numerateur YB YA sub def
		/angleDirectionAB numerateur denominateur Atan def
		/XD StartArrow angleDirectionAB cos mul XA add def
		/YD StartArrow angleDirectionAB sin mul YA add def
		/XF XD LengthArrow angleDirectionAB cos mul add def
		/YF YD LengthArrow angleDirectionAB sin mul add def
		XD YD ){ArrowStart}
	\pnode(! XF YF){ArrowEnd}
	\psset{arrows=->}
	\psline[#1](ArrowStart)(ArrowEnd)%
}}
%
% draw a line (===) outside: #2-----#3=======#4
%
\def\psOutLine{\@ifnextchar[{\pst@ToDrawOut}{\pst@ToDrawOut[]}}
\def\pst@ToDrawOut[#1](#2)(#3)#4{{%
	\setkeys{psset}{#1}%
	\pst@getcoor{#2}\pst@tempa
	\pst@getcoor{#3}\pst@tempb
	\pnode(!%
		/LengthArrow \psk@ThreeDplot@length\space def
		\pst@tempa /YA exch \pst@number\psyunit div def
		/XA exch \pst@number\psxunit div def
		\pst@tempb /YB exch \pst@number\psyunit div def
		/XB exch \pst@number\psxunit div def
		/denominateur XB XA sub def
		/numerateur YB YA sub def
		/angleDirectionAB numerateur denominateur Atan def
		/Xend XB LengthArrow angleDirectionAB cos mul add def
		/Yend YB LengthArrow angleDirectionAB sin mul add def
		Xend Yend){#4}
	\psline[#1](#3)(#4)
}}
%
% draw a line (===) before: #4========#2-----#3
%
\def\psBeforeLine{\@ifnextchar[{\pst@BeforeLine}{\pst@BeforeLine[]}}
\def\pst@BeforeLine[#1](#2)(#3)#4{{%
	\setkeys{psset}{#1}%
	\pst@getcoor{#2}\pst@tempa
	\pst@getcoor{#3}\pst@tempb
	\pnode(!%
		/LengthArrow \psk@ThreeDplot@length\space def
		\pst@tempa /YA exch \pst@number\psyunit div def
		/XA exch \pst@number\psxunit div def
		\pst@tempb /YB exch \pst@number\psyunit div def
		/XB exch \pst@number\psxunit div def
		/denominateur XB XA sub def
		/numerateur YB YA sub def
		/angleDirectionAB numerateur denominateur Atan def
		/Xstart XA LengthArrow angleDirectionAB cos mul sub def
		/Ystart YA LengthArrow angleDirectionAB sin mul sub def
		Xstart Ystart){#4}
	\psline[#1](#4)(#2)%
}}
%
% intersection de deux droites
% 2 juillet 2001/ rewritten 2003-01-27 Herbert
%
\def\ABinterCD(#1)(#2)(#3)(#4)#5{%
    \pst@getcoor{#1}\pst@tempa
    \pst@getcoor{#2}\pst@tempb
    \pst@getcoor{#3}\pst@tempc
    \pst@getcoor{#4}\pst@tempd
\pnode(!%
    /YA \pst@tempa exch pop \pst@number\psyunit div def
    /XA \pst@tempa pop \pst@number\psxunit div def
    /YB \pst@tempb exch pop \pst@number\psyunit div def
    /XB \pst@tempb pop \pst@number\psxunit div def
    /YC \pst@tempc exch pop \pst@number\psyunit div def
    /XC \pst@tempc pop \pst@number\psxunit div def
    /YD \pst@tempd exch pop \pst@number\psyunit div def
    /XD \pst@tempd pop \pst@number\psxunit div def
    /dY1 YB YA sub def
    /dX1 XB XA sub def
    /dY2 YD YC sub def
    /dX2 XD XC sub def
    dX1 abs 0.01 lt {
	/m2 dY2 dX2 div def
	XA dup XC sub m2 mul YC add 
    }{
	dX2 abs 0.01 lt {
	    /m1 dY1 dX1 div def
	    XC dup XA sub m1 mul YA add 
	}{%
	    /m1 dY1 dX1 div def
	    /m2 dY2 dX2 div def
	    m1 XA mul m2 XC mul sub YA sub YC add m1 m2 sub div dup
	    XA sub m1 mul YA add 
	} ifelse
    } ifelse ){#5}
}
%
% draw a parallel line
%     #2---------#3
%         #4----------#5(new)  
\def\Parallel{\@ifnextchar[{\pst@Parallel}{\pst@Parallel[]}}
\def\pst@Parallel[#1](#2)(#3)(#4)#5{{%
	\setkeys{psset}{#1}%
	\pst@getcoor{#2}\pst@tempa
	\pst@getcoor{#3}\pst@tempb
	\pst@getcoor{#4}\pst@tempc
	\pnode(!%
		/LengthArrow \psk@ThreeDplot@length\space def
		\pst@tempa /YA exch \pst@number\psyunit div def
		/XA exch \pst@number\psxunit div def
		\pst@tempb /YB exch \pst@number\psyunit div def
		/XB exch \pst@number\psxunit div def
		\pst@tempc /YC exch \pst@number\psyunit div def
		/XC exch \pst@number\psxunit div def
		/denominateur XB XA sub def
		/numerateur YB YA sub def
		/angleDirectionAB numerateur denominateur Atan def
		/XstartParallel XC LengthArrow angleDirectionAB cos mul add def
		/YstartParallel YC LengthArrow angleDirectionAB sin mul add def
		XstartParallel YstartParallel){#5}
	\psline[#1](#4)(#5)
}}
%
% arrowLine[options](A)(B){n}
% #2---->---->---->---->----#3  #4-arrows inside
\def\arrowLine{\@ifnextchar[{\pst@arrowLine}{\pst@arrowLine[]}}
\def\pst@arrowLine[#1](#2)(#3)#4{{%
	\setkeys{psset}{arrowsize=4pt,arrows=->}% the defaults
	\setkeys{psset}{#1}%
	\def\pst@ThreeDplot@n{#4}
	\pst@getcoor{#2}\pst@tempa
	\pst@getcoor{#3}\pst@tempb
	\pnode(!%
	    	/YA \pst@tempa exch pop \pst@number\psyunit div def
		/XA \pst@tempa pop \pst@number\psxunit div def
		/YB \pst@tempb exch pop \pst@number\psyunit div def
		/XB \pst@tempb pop \pst@number\psxunit div def
		/dY YB YA sub \pst@ThreeDplot@n\space 1 add div def
		/dX XB XA sub \pst@ThreeDplot@n\space 1 add div def
		/Alpha dY dX atan def
		/dYOffset \psk@ThreeDplot@arrowOffset\space Alpha sin mul def
		/dXOffset \psk@ThreeDplot@arrowOffset\space Alpha cos mul def
		XA YA ){tempArrowC}
	\multido{\i=1+1}{#4}{%
		\pnode(!%
			XA dX \i\space mul add dXOffset add
			YA dY \i\space mul add dYOffset add){tempArrowB}
		\psline(tempArrowC)(tempArrowB)
		\pnode(tempArrowB){tempArrowC}
    	}
	\psline[arrows=-](tempArrowB)(#3)
}}
%
%   #1------#3------#2
\def\nodeBetween(#1)(#2)#3{%    Herbert 2003/01/05
    \pst@getcoor{#1}\pst@tempa
    \pst@getcoor{#2}\pst@tempb
    \pnode(!%
	/XA \pst@tempa pop \pst@number\psxunit div def
	/YA \pst@tempa exch pop \pst@number\psyunit div def
	/XB \pst@tempb pop \pst@number\psxunit div def
	/YB \pst@tempb exch pop \pst@number\psyunit div def
	XB XA add 2 div YB YA add 2 div){#3}
}
%
% rotateNode(A)
% (A) the node
% #2  the angle
% Herbert Voss <voss@perce.de> 2003-01-26
\def\rotateNode{\pst@rotateNode}
\def\pst@rotateNode(#1)#2{{%
    \pst@getcoor{#1}\pst@tempa
    \def\pst@ThreeDplot@angle{#2}	% the rotating angle
    \pnode(!%
    	/YA \pst@tempa exch pop \pst@number\psyunit div def
	/XA \pst@tempa pop \pst@number\psxunit div def
	YA 0 eq XA 0 eq and {0 0}{
	    /r XA dup mul YA dup mul add sqrt def
	    /AlphaOld YA XA atan def
	    /AlphaNew AlphaOld \pst@ThreeDplot@angle\space add def
	    r AlphaNew cos mul r AlphaNew sin mul
	} ifelse ){temp}
    \pnode(temp){#1}
}}
%
\def\rotateTriangle{\pst@rotateTriangle}
\def\pst@rotateTriangle(#1)(#2)(#3)#4{{%
    \rotateNode(#1){#4}
    \rotateNode(#2){#4}
    \rotateNode(#3){#4}
}}
%
\def\rotateFrame{\pst@rotateFrame}
\def\pst@rotateFrame(#1)(#2)(#3)(#4)#5{{%
    \rotateNode(#1){#5}
    \rotateNode(#2){#5}
    \rotateNode(#3){#5}
    \rotateNode(#4){#5}
}}
\catcode`\@=\PstAtCode\relax
%
%% END: pst-3dplot.tex
\endinput

%% CHANGE LOG %%
%
% 1.30	new written macros
% 1.2d	added option none for dotstyle
% 1.2c	added sperical coordinates
% 1.2b	bugfix for adding vectors with decinmal length
% 1.2a	disable the loading of pstcol.sty


==> pst-vue3d.tex <==

%% This is file `pst-vue3d.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pst-vue3d.tex'
%%
%% Manuel Luque <Mluque5130@aol.com> (France)
%%
%% 2003/12/21
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-vue3d' is a PSTricks package to define 3d views
%% ChangeLog (at end)
%%
\def\fileversion{1.0g}%
\def\filedate{2003/12/21}%
\message{`PST-VUE3D v\fileversion, \filedate\space (Manuel LUQUE)}%
\csname PSTVueTroisDLoaded\endcsname
\let\PSTVueTroisDLoaded\endinput
% Require PSTricks and pst-node packages
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTnodesLoaded\endinput\else\input pst-node.tex\fi
% DPC interface to the `keyval' package (until keyval based version of PSTricks)
\input pst-key.tex
%
\edef\PstAtCode{\the\catcode`\@} \catcode`\@=11\relax
\SpecialCoor

\pstheader{3D.pro}
%%%%
\SpecialCoor
\makeatletter
\define@key{psset}{scale}{\edef\psk@TroisD@scale{#1}} % echelle
\define@key{psset}{RotX}{\edef\psk@TroisD@RotX{#1}} % rotation autour de Ox en degrés
\define@key{psset}{RotY}{\edef\psk@TroisD@RotY{#1}} % rotation autour de Oy en degrés
\define@key{psset}{RotZ}{\edef\psk@TroisD@RotZ{#1}} % rotation autour de OZ en degrés
\define@key{psset}{A}{\edef\psk@TroisD@A{#1}} % double  d'une arête du parallèlépipède
\define@key{psset}{B}{\edef\psk@TroisD@B{#1}} % double  d'une arête du parallèlépipède
\define@key{psset}{C}{\edef\psk@TroisD@C{#1}} % double  de l'arête du parallèlépipède
\define@key{psset}{Rtetraedre}{\edef\psk@TroisD@Rtetraedre{#1}} % Rayon du cercle tétraèdre
\define@key{psset}{ColorFaceA}{\edef\psk@TroisD@TetraedreColorFaceA{#1}} % couleur de la face A du tétraèdre
\define@key{psset}{ColorFaceB}{\edef\psk@TroisD@TetraedreColorFaceB{#1}} % couleur de la face B du tétraèdre
\define@key{psset}{ColorFaceC}{\edef\psk@TroisD@TetraedreColorFaceC{#1}} % couleur de la face C du tétraèdre
\define@key{psset}{ColorFaceD}{\edef\psk@TroisD@TetraedreColorFaceD{#1}} % couleur de la face D du tétraèdre
\define@key{psset}{ColorFaceE}{\edef\psk@TroisD@TetraedreColorFaceE{#1}} % couleur de la face D du tétraèdre
\define@key{psset}{fracHeight}{\edef\psk@TroisD@fracHeight{#1}} % fraction de la hauteur du cone
\define@key{psset}{fracHcone}{\edef\psk@TroisD@fracHeight{#1}} % for compatibility
%
\define@key{psset}{normaleLongitude}{\edef\psk@TroisD@normaleLongitude{#1}} % coordonnées angulaires de la normale
\define@key{psset}{normaleLatitude}{\edef\psk@TroisD@normaleLatitude{#1}} % coordonnées angulaires de la normale
\define@key{psset}{pas}{\edef\psk@TroisD@pas{#1}} % en cm résolution du tracé
\define@key{psset}{grille}{\edef\psk@TroisD@grille{#1}} % Pas de la grille en cm
%
\define@key{psset}{THETA}{\edef\psk@TroisD@Theta{#1}}
\define@key{psset}{PHI}{\edef\psk@TroisD@Phi{#1}}
\define@key{psset}{DeltaTHETA}{\edef\psk@TroisD@DeltaTheta{#1}}
\define@key{psset}{DeltaPHI}{\edef\psk@TroisD@DeltaPhi{#1}}
\define@key{psset}{PortionSphereTHETA}{\edef\psk@TroisD@PortionSphereTHETA{#1}}
\define@key{psset}{PortionSpherePHI}{\edef\psk@TroisD@PortionSpherePHI{#1}}
\define@key{psset}{PhiCercle}{\edef\psk@TroisD@PhiCercle{#1}}
\define@key{psset}{ThetaMeridien}{\edef\psk@TroisD@ThetaMeridien{#1}}
\define@key{psset}{Dobs}{\edef\psk@TroisD@Dobs{#1}}
\define@key{psset}{Decran}{\edef\psk@TroisD@Ecran{#1}}
%
\setkeys{psset}{THETA=30,PHI=10,%
	Dobs=100,Decran=10,%
	normaleLongitude=45,%
	normaleLatitude=45,%
	PhiCercle=0,%
	ThetaMeridien=0,%
	pas=1,%
	grille=10,%
	scale=1,%
	RotX=0,RotY=0,RotZ=0,%
	A=10,B=10,C=10,%
	Rtetraedre=5,%
	ColorFaceD=cyan,ColorFaceA=magenta,ColorFaceB=red,%
	ColorFaceC=blue,ColorFaceE=yellow,%
	fracHeight=1,%
	DeltaTHETA=10,DeltaPHI=10,%
	PortionSphereTHETA=0,PortionSpherePHI=0}
% ajout du 28 août 2003
% colorier au choix les faces du cube
\define@key{psset}{CubeColorFaceOne}{\edef\psk@TroisD@CubeColorFaceOne{#1}} % couleur de la face 1 du cube
\define@key{psset}{CubeColorFaceTwo}{\edef\psk@TroisD@CubeColorFaceTwo{#1}} % couleur de la face 2 du cube
\define@key{psset}{CubeColorFaceThree}{\edef\psk@TroisD@CubeColorFaceThree{#1}} % couleur de la face 3 du cube
\define@key{psset}{CubeColorFaceFour}{\edef\psk@TroisD@CubeColorFaceFour{#1}} % couleur de la face 4 du cube
\define@key{psset}{CubeColorFaceFive}{\edef\psk@TroisD@CubeColorFaceFive{#1}} % couleur de la face 5 du cube
\define@key{psset}{CubeColorFaceSix}{\edef\psk@TroisD@CubeColorFaceSix{#1}} % couleur de la face 6 du cube
\setkeys{psset}{CubeColorFaceOne= 1 1 0 ,
                CubeColorFaceTwo= 0.9 0.9 0 ,
                CubeColorFaceThree= 0.8 0.8 0 ,
                CubeColorFaceFour= 0.7 0.7 0 ,
                CubeColorFaceFive= 0.6 0.6 0 ,
                CubeColorFaceSix= 0.5 0.5 0 }
% fin 28 août 2003
% ajout 27 octobre 2003
\newif\ifPst@cubeInside
\define@key{psset}{CubeInside}[false]{\@nameuse{Pst@cubeInside#1}}
\setkeys{psset}{CubeInside=false}
% hv 2003-12-20
\newif\ifPst@SphericalCoor
\define@key{psset}{SphericalCoor}[true]{\@nameuse{Pst@SphericalCoor#1}}
\setkeys{psset}{SphericalCoor=false}
%
\def\variablesTroisD{%
 0 0 translate
    /reduction \psk@TroisD@scale\space def
    /RotX \psk@TroisD@RotX\space def
    /RotY \psk@TroisD@RotY\space def
    /RotZ \psk@TroisD@RotZ\space def
    /A \psk@TroisD@A\space def
    /B \psk@TroisD@B\space def
    /C \psk@TroisD@C\space def
    /RayonBaseTetraedre \psk@TroisD@Rtetraedre\space def
    /fracHeight \psk@TroisD@fracHeight\space def
    /Rpoint A 4 div def
    /nTheta \psk@TroisD@normaleLongitude\space def
    /nPhi \psk@TroisD@normaleLatitude\space def
    /S1 \psk@TroisD@normaleLongitude\space sin def
    /C1 \psk@TroisD@normaleLongitude\space cos def
    /S2 \psk@TroisD@normaleLatitude\space sin def
    /C2 \psk@TroisD@normaleLatitude\space cos def
    /THETA \psk@TroisD@Theta\space def
    /PHI \psk@TroisD@Phi\space def
    /dTHETA \psk@TroisD@DeltaTheta\space def
    /dPHI \psk@TroisD@DeltaPhi\space def
    /psTHETA \psk@TroisD@PortionSphereTHETA\space def
    /psPHI \psk@TroisD@PortionSpherePHI\space def
    /PhiCercle \psk@TroisD@PhiCercle\space def
    /ThetaMeridien \psk@TroisD@ThetaMeridien\space def
    /Dobs \psk@TroisD@Dobs\space def
    /DScreen \psk@TroisD@Ecran\space def
    /Sin1 THETA sin def
    /Sin2 PHI sin def
    /Cos1 THETA cos def
    /Cos2 PHI cos def
    /Cos1Sin2 Cos1 Sin2 mul def
    /Sin1Sin2 Sin1 Sin2 mul def
    /Cos1Cos2 Cos1 Cos2 mul def
    /Sin1Cos2 Sin1 Cos2 mul def
    /XpointVue Dobs Cos1Cos2 mul def
    /YpointVue Dobs Sin1Cos2 mul def
    /ZpointVue Dobs Sin2 mul def
    /M11 RotZ cos RotY cos mul def
    /M12 RotZ cos RotY sin mul RotX sin mul
         RotZ sin RotX cos mul sub def
    /M13 RotZ cos RotY sin mul RotX cos mul
         RotZ sin RotX sin mul add def
    /M21 RotZ sin RotY cos mul def
    /M22 RotZ sin RotY sin RotX sin mul mul
         RotZ cos RotX cos mul add def
    /M23 RotZ sin RotY sin mul RotX cos mul
         RotZ cos RotX sin mul sub def
    /M31 RotY sin neg def
    /M32 RotX sin RotY cos mul def
    /M33 RotX cos RotY cos mul def
 }%
% hv 2003-12-20
% -------------- Utilities -----------------
\def\face{%
	\pscurve(1;160)(0.8;180)(1;200)
	\pscustom{\gsave\psarc(0,0){1}{165}{195}
		\pscurve(1;195)(0.85;180)(1;165)
		\fill[fillstyle=solid,fillcolor=blue]\grestore}
	\pscurve[linewidth=.4pt](1;195)(0.85;180)(1;165)
	\bgroup
		\psset{linewidth=2pt}
		\psarc(0,1){1}{180}{270}
		\psarc(0,-1){1}{90}{180}
	\egroup
	\psarc(0,0){1}{150}{210}
	\psset{linewidth=4pt,linecolor=gray}%
	\pscurve(-.5,3.5)(-1,3)(-1.2,2.5)(-1.3,2)(-1.4,1)(-1.35,0.5)%
		(-1.2,-.2)(-1.35,-.5)(-1.4,-1)(-1.5,-1.5)(-1.8,-2)(-1.8,-2.3)%
		(-1.65,-2.5)(-1.35,-2.55)(-.95,-2.8)(-.95,-3.35)(-1,-3.65)(-.8,-4)(-.4,-4.1)
	\pscurve(-.8,-4)(-.8,-4.2)(-.5,-4.5)(-.4,-5)(-.25,-5.5)(0,-5.8)(.5,-6)%
}
\def\eye{%
    \psarc[linewidth=2pt](0,2.5){2.5}{215}{270}%
    \psarc[linewidth=2pt](0,-2.5){2.5}{90}{140}%
    \psarc(-2.5,0){1}{-30}{30}%
    \psarc(0,0){1.75}{160}{200}
    \psclip{%
	\pscircle[linestyle=none](0,0){1.75}}
    \pscircle[fillstyle=solid,fillcolor=lightgray](-2.5,0){0.9}
    \endpsclip%
}
%
% -------------- Basic Macros --------------
%
% hv 2003
\def\AxesThreeD{\@ifnextchar[{\AxesThreeD@i}{\AxesThreeD@i[]}}
\def\AxesThreeD@i[#1](#2){{%
	\setkeys{psset}{#1}%
	\AxesThreeD@ii#2,@comma*\relax%
}}
\def\AxesThreeD@ii#1,#2*{%
	\def\@tempa{#2}\def\@tempb{@comma}%
	\ifx\@tempa\@tempb% only one value
		\AxesThreeD@iii#1,#2\else\AxesThreeD@iv#1,#2\relax%
	\fi%
}
\def\AxesThreeD@iii#1,#2\relax{%
	\AxesThreeD@iv#1,#1,#1,#1\relax%
}
\def\AxesThreeD@iv#1,#2,#3,#4\relax{{%
	\pNodeThreeD(0,0,0){O}%
	\pNodeThreeD(0,0,#3){Z}\pNodeThreeD(#1,0,0){X}\pNodeThreeD(0,#2,0){Y}%
	\psline{->}(O)(Z)\psline{->}(O)(X)\psline{->}(O)(Y)%
	\uput[0](Z){\small Z}\uput[90](X){\small X}\uput[0](Y){\small Y}%
}}
%
% hv 2003
\def\showCoorThreeD{\@ifnextchar[{\showCoorThreeD@i}{\pshowCoorThreeD@i[]}}
\def\showCoorThreeD@i[#1](#2){{%
	\psset{linestyle=dashed}
	\setkeys{psset}{#1}
	\showCoorThreeD@ii#2,@comma*\relax
}}
\def\showCoorThreeD@ii#1,#2*{%
	\def\@tempa{#2}\def\@tempb{@comma}%
	\ifx\@tempa\@tempb%
		\showCoorThreeD@iii#1;#2\else\showCoorThreeD@iv#1,#2\relax%
	\fi%
}
\def\showCoorThreeD@iii#1;#2;#3;#4\relax{%
	\psline(!
		\variablesTroisD
		/Radius #1 def
		/longitude #2 def
		/latitude #3 def
		/Zcote Radius latitude sin mul def
		/Xabscisse Radius longitude cos mul latitude cos mul def
		/Yordonnee Radius longitude sin mul latitude cos mul def
		tx@3DDict begin
			formulesTroisD
			Xi reduction mul Yi reduction mul
		end)(!
		/Zcote 0 def
		tx@3DDict begin
			formulesTroisD
			Xi reduction mul Yi reduction mul
		end)
	\psline(!
		/Zcote 0 def
		/Xabscisse Radius longitude cos mul latitude cos mul def
		/Yordonnee Radius longitude sin mul latitude cos mul def
		tx@3DDict begin
			formulesTroisD
			Xi reduction mul Yi reduction mul
		end)(!
		/Zcote 0 def
		/Yordonnee 0 def
		tx@3DDict begin
			formulesTroisD
			Xi reduction mul Yi reduction mul
		end)
	\psline(!
		/Zcote 0 def
		/Xabscisse Radius longitude cos mul latitude cos mul def
		/Yordonnee Radius longitude sin mul latitude cos mul def
		tx@3DDict begin
			formulesTroisD
			Xi reduction mul Yi reduction mul
		end)(!
		/Zcote 0 def
		/Xabscisse 0 def
		tx@3DDict begin
			formulesTroisD
			Xi reduction mul Yi reduction mul
		end)
}
\def\showCoorThreeD@iv#1,#2,#3,#4\relax{%
%	\qdisk(P){1pt}
	\LineThreeD(#1,#2,#3)(#1,#2,0)
	\LineThreeD(#1,#2,0)(#1,0,0)
	\LineThreeD(#1,#2,0)(0,#2,0)
}
%
%
\def\CubeThreeD{\pst@object{CubeThreeD}}
\def\CubeThreeD@i{\@ifnextchar[{\CubeThreeD@do}{\CubeThreeD@do[]}}
\def\CubeThreeD@do[#1](#2,#3,#4){{%
    \pst@killglue
    \setkeys{psset}{#1}%
    \begin@ClosedObj
    \addto@pscode{%
	\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
	\ifPst@cubeInside
	    /Condition { ge } def
	\else
	    /Condition {le } def
	\fi
	/CubeColorFaceOne {\psk@TroisD@CubeColorFaceOne} def
	/CubeColorFaceTwo {\psk@TroisD@CubeColorFaceTwo} def
	/CubeColorFaceThree {\psk@TroisD@CubeColorFaceThree} def
	/CubeColorFaceFive {\psk@TroisD@CubeColorFaceFive} def
	/CubeColorFaceFour {\psk@TroisD@CubeColorFaceFour} def
	/CubeColorFaceSix {\psk@TroisD@CubeColorFaceSix} def
	tx@3DDict begin
	    /Condition1 {PS1 0 le } def
	    Cube
	end
    }% fin du code ps
    \end@ClosedObj%
}}
%
\def\DieThreeD{\pst@object{DieThreeD}}
\def\DieThreeD@i{\@ifnextchar[{\DieThreeD@do}{\DieThreeD@do[]}}
\def\DieThreeD@do[#1](#2,#3,#4){{%
% (#2,#3,#4) coordonnées du centre
    \pst@killglue
    \setkeys{psset}{#1}%
    \begin@ClosedObj
	\addto@pscode{%
	    \variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
	    \ifPst@cubeInside
		/Condition { ge } def
	    \else
		/Condition {le } def
	    \fi
	    /CubeColorFaceOne {\psk@TroisD@CubeColorFaceOne} def
	    /CubeColorFaceTwo {\psk@TroisD@CubeColorFaceTwo} def
	    /CubeColorFaceThree {\psk@TroisD@CubeColorFaceThree} def
	    /CubeColorFaceFive {\psk@TroisD@CubeColorFaceFive} def
	    /CubeColorFaceFour {\psk@TroisD@CubeColorFaceFour} def
	    /CubeColorFaceSix {\psk@TroisD@CubeColorFaceSix} def
	    tx@3DDict begin
		Cube
		PointsDie
	    end
	}% fin du code ps
    \end@ClosedObj%
}}
%
\def\SphereThreeD{\pst@object{SphereThreeD}}
\def\SphereThreeD@i{\@ifnextchar[{\SphereThreeD@do}{\SphereThreeD@do[]}}
\def\SphereThreeD@do[#1](#2,#3,#4)#5{{%
% (#2,#3,#4) coordonnées du centre
% #5 rayon
    \pst@killglue
    \setkeys{psset}{#1}%
    \begin@ClosedObj
	\addto@pscode{%
	    \variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
	    reduction reduction scale
	    /Rsphere #5 def
	    /increment 10 def
	    tx@3DDict begin
			/condition {PSfacette 0 le} def
			/departPhi -90 def
			MaillageSphere
	    end
	}% fin du code ps
	\showpointsfalse
	\end@ClosedObj%
}}
% % fin de la commande PSTricks
%
% 2décembre 2002
%
\def\SphereInverseThreeD{\pst@object{SphereInverseThreeD}}
\def\SphereInverseThreeD@i{\@ifnextchar[{\SphereInverseThreeD@do}{\SphereInverseThreeD@do[]}}
\def\SphereInverseThreeD@do[#1](#2,#3,#4)#5{{%
% (#2,#3,#4) coordonnées du centre
% #5 rayon
    \pst@killglue
    \setkeys{psset}{#1}%
    \begin@ClosedObj
	\addto@pscode{%
	    \variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
	    reduction reduction scale
	    /Rsphere #5 def
	    /increment 10 def
	    tx@3DDict begin
		/condition {PSfacette 0 ge} def
		/departPhi -90 def
		MaillageSphere
	    end
	}% fin du code ps
	\showpointsfalse
	\end@ClosedObj%
}}
% % fin de la commande PSTricks
% fin 2 décembre 2002
%
\def\SphereCercleThreeD{\pst@object{SphereCercleThreeD}}
\def\SphereCercleThreeD@i{\@ifnextchar[{\SphereCercleThreeD@do}{\SphereCercleThreeD@do[]}}
\def\SphereCercleThreeD@do[#1](#2,#3,#4)#5{{%
% (#2,#3,#4) coordonnées du centre
% #5 rayon
    \pst@killglue
    \setkeys{psset}{#1}%
    \begin@ClosedObj
	\addto@pscode{%
	    \variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
	    reduction reduction scale
	    /Rsphere #5 def
	    tx@3DDict begin
	    0 2 360 {
		/ThetaEquateur exch def
		/Xpoint Rsphere ThetaEquateur cos mul PhiCercle cos mul def
		/Ypoint Rsphere ThetaEquateur sin mul PhiCercle cos mul def
		/Zpoint Rsphere PhiCercle sin mul def
		CalculsPointsAfterTransformations
% rayon de las sphère (normale)
		/nXfacette Xabscisse CX sub def
		/nYfacette Yordonnee CY sub def
		/nZfacette Zcote CZ sub def
% rayon vers point de vue
		/RXvue Xabscisse XpointVue sub def
		/RYvue Yordonnee YpointVue sub def
		/RZvue Zcote ZpointVue sub def
% test de visibilité
		/PSPoint RXvue nXfacette mul
		    RYvue nYfacette mul add
		    RZvue nZfacette mul add
		def
		PSPoint 0 le{
		    newpath
			CalcCoordinates
			0.5 0 360 arc
		    closepath
		    fill
		} if
%lineto
	    } for
	    end
	}% fin du code ps
    \showpointsfalse
    \end@ClosedObj%
}}
%
%
\def\SphereMeridienThreeD{\pst@object{SphereMeridienThreeD}}
\def\SphereMeridienThreeD@i{\@ifnextchar[{\SphereMeridienThreeD@do}{\SphereMeridienThreeD@do[]}}
\def\SphereMeridienThreeD@do[#1](#2,#3,#4)#5{{%
% (#2,#3,#4) coordonnées du centre
% #5 rayon
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
	\addto@pscode{%
		\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
		reduction reduction scale
		/Rsphere #5 def
		tx@3DDict begin
0 2 360 {
    /PhiCercle exch def
    /Xpoint Rsphere ThetaMeridien cos mul PhiCercle cos mul def
    /Ypoint Rsphere ThetaMeridien sin mul PhiCercle cos mul def
    /Zpoint Rsphere PhiCercle sin mul def
CalculsPointsAfterTransformations
% rayon de las sphère (normale)
    /nXfacette Xabscisse CX sub def
    /nYfacette Yordonnee CY sub def
    /nZfacette Zcote CZ sub def
% rayon vers point de vue
    /RXvue Xabscisse XpointVue sub def
    /RYvue Yordonnee YpointVue sub def
    /RZvue Zcote ZpointVue sub def
% test de visibilité
    /PSPoint RXvue nXfacette mul
    RYvue nYfacette mul add
    RZvue nZfacette mul add
    def
PSPoint 0 le{
	newpath
    CalcCoordinates
	0.5 0 360 arc
closepath
fill
} if
%lineto
} for
end
 }% fin du code ps
\showpointsfalse
\end@ClosedObj
}}
%
\def\CylindreThreeD{\pst@object{CylindreThreeD}}
\def\CylindreThreeD@i{\@ifnextchar[{\CylindreThreeD@do}{\CylindreThreeD@do[]}}
\def\CylindreThreeD@do[#1](#2,#3,#4)#5#6{{%
% Le centre de la base sera placé avec
% (#2,#3,#4) les paramètres CX,CY et CZ
% #5 rayon
% #6 hauteur
% on peut ensuite faire tourner le cylindre
% avec RotX, RotY et RotZ
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
	\addto@pscode{%
		\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
		reduction reduction scale
		/Rcylindre #5 def
		/Hcylindre #6 def
		/incrementANGLE 10 def
		/incrementHAUTEUR Hcylindre 5 div def
		tx@3DDict begin
			CylinderThreeD
		end
	}% fin du code ps
	\showpointsfalse
\end@ClosedObj
}}% % fin de la commande PSTricks
%
% hv 2003-12-18
\def\LineThreeD{\@ifnextchar[{\LineThreeD@i}{\LineThreeD@i[]}}
\def\LineThreeD@i[#1](#2,#3,#4)(#5,#6,#7){{%
% (#2,#3,#4) coordonnées du point1
% (#5,#6,#7) coordonnées du point2
	\pst@killglue
	\psset{#1}
	\pNodeThreeD(#2,#3,#4){tempNodeA}
	\pNodeThreeD(#5,#6,#7){tempNodeB}
	\psline(tempNodeA)(tempNodeB)
}}
%
% hv 2003-12-17
\def\pNodeThreeD{\@ifnextchar[{\pNodeThreeD@i}{\pNodeThreeD@i[]}}
% point can be in cartesian (x,y,z) or sphere coordinates (r;phi;theta)
\def\pNodeThreeD@i[#1](#2)#3{{%
	\setkeys{psset}{#1}
	\edef\@NodeNameThreeD{#3}
	\pNodeThreeD@ii#2,@comma*\relax
}}
\def\pNodeThreeD@ii#1,#2*{%
	\def\@tempa{#2}\def\@tempb{@comma}%
	\ifx\@tempa\@tempb%
		\pNodeThreeD@iii#1;#2\else\pNodeThreeD@iv#1,#2\relax%
	\fi%
}
\def\pNodeThreeD@iii#1;#2;#3;#4\relax{%
	\pnode(!
		\variablesTroisD
		/Radius #1 def
		/longitude #2 def
		/latitude #3 def
		/Zcote Radius latitude sin mul def
		/Xabscisse Radius longitude cos mul latitude cos mul def
		/Yordonnee Radius longitude sin mul latitude cos mul def
		tx@3DDict begin
			formulesTroisD
			Xi reduction mul Yi reduction mul
		end){\@NodeNameThreeD}
}
\def\pNodeThreeD@iv#1,#2,#3,#4\relax{%
	\pnode(!
		\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #1 def
			/longitude #2 def
			/latitude #3 def
			/Zcote Radius latitude sin mul def
			/Xabscisse Radius longitude cos mul latitude cos mul def
			/Yordonnee Radius longitude sin mul latitude cos mul def
		\else
			/Zcote #3 def
			/Xabscisse #1 def
			/Yordonnee #2 def
		\fi
		tx@3DDict begin
			formulesTroisD
			Xi reduction mul Yi reduction mul
		end){\@NodeNameThreeD}%
}
%
%
\def\TetraedreThreeD{\pst@object{TetraedreThreeD}}
\def\TetraedreThreeD@i{\@ifnextchar[{\TetraedreThreeD@do}{\TetraedreThreeD@do[]}}
\def\TetraedreThreeD@do[#1](#2,#3,#4){{%
    \pst@killglue
    \setkeys{psset}{#1}%
    \begin@ClosedObj
	\addto@pscode{%
	    \variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
	    tx@3DDict begin
			Tetraedre
	    end
	}% fin du code ps
    \end@ClosedObj
}}
%
%
% pyramide
%
\def\FaceSAB{\pst@object{FaceSAB}}
\def\FaceSAB@i{\@ifnextchar[{\FaceSAB@do}{\FaceSAB@do[]}}
\def\FaceSAB@do[#1](#2,#3,#4)#5{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
    \addto@pscode{%
	\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
	/Hpyramide #5 def
	tx@3DDict begin
	    SommetsPyramide
	    PSAB 0 le { %
		reduction reduction scale
		newpath
		1 setlinejoin
		/Xabscisse XS 1 fracHeight sub XA XS sub mul add def
		/Yordonnee YS 1 fracHeight sub YA YS sub mul add def
		/Zcote ZS CZ sub fracHeight mul CZ add def
		CalcCoordinates
		moveto
		/Xabscisse XA def
		/Yordonnee YA def
		/Zcote ZA def
		CalcCoordinates
		lineto
		/Xabscisse XB def
		/Yordonnee YB def
		/Zcote ZB def
		CalcCoordinates
		lineto
		/Xabscisse XS 1 fracHeight sub XB XS sub mul add def
		/Yordonnee YS 1 fracHeight sub YB YS sub mul add def
		/Zcote ZS CZ sub fracHeight mul CZ add def
		CalcCoordinates
		lineto
		closepath
	    } if
	end
    }% fin du code ps
\end@ClosedObj
}}
%
\def\FaceSBC{\pst@object{FaceSBC}}
\def\FaceSBC@i{\@ifnextchar[{\FaceSBC@do}{\FaceSBC@do[]}}
\def\FaceSBC@do[#1](#2,#3,#4)#5{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
    \addto@pscode{%
	\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
	/Hpyramide #5 def
	tx@3DDict begin
	    SommetsPyramide
	    PSBC 0 le { %
		reduction reduction scale
		newpath
		1 setlinejoin
		/Xabscisse XS 1 fracHeight sub XB XS sub mul add def
		/Yordonnee YS 1 fracHeight sub YB YS sub mul add def
		/Zcote ZS CZ sub fracHeight mul CZ add def
		CalcCoordinates
		moveto
		/Xabscisse XB def
		/Yordonnee YB def
		/Zcote ZB def
		CalcCoordinates
		lineto
		/Xabscisse XC def
		/Yordonnee YC def
		/Zcote ZC def
		CalcCoordinates
		lineto
		/Xabscisse XS 1 fracHeight sub XC XS sub mul add def
		/Yordonnee YS 1 fracHeight sub YC YS sub mul add def
		/Zcote ZS CZ sub fracHeight mul CZ add def
		CalcCoordinates
		lineto
		closepath
	    } if
	end
    }% fin du code ps
\end@ClosedObj
}}
%
%
\def\FaceSCD{\pst@object{FaceSCD}}
\def\FaceSCD@i{\@ifnextchar[{\FaceSCD@do}{\FaceSCD@do[]}}
\def\FaceSCD@do[#1](#2,#3,#4)#5{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
    \addto@pscode{%
	\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
	/Hpyramide #5 def
	tx@3DDict begin
	    SommetsPyramide
	    PSCD 0 le { %
    		reduction reduction scale
		newpath
		1 setlinejoin
		/Xabscisse XS 1 fracHeight sub XC XS sub mul add def
		/Yordonnee YS 1 fracHeight sub YC YS sub mul add def
		/Zcote ZS CZ sub fracHeight mul CZ add def
		CalcCoordinates
		moveto
		/Xabscisse XC def
		/Yordonnee YC def
		/Zcote ZC def
		CalcCoordinates
		lineto
		/Xabscisse XD def
		/Yordonnee YD def
		/Zcote ZD def
		CalcCoordinates
		lineto
		/Xabscisse XS 1 fracHeight sub XD XS sub mul add def
		/Yordonnee YS 1 fracHeight sub YD YS sub mul add def
		/Zcote ZS CZ sub fracHeight mul CZ add def
		CalcCoordinates
		lineto
		closepath
	    } if
	end
    }% fin du code ps
\end@ClosedObj
}}
%
\def\FaceSDA{\pst@object{FaceSDA}}
\def\FaceSDA@i{\@ifnextchar[{\FaceSDA@do}{\FaceSDA@do[]}}
\def\FaceSDA@do[#1](#2,#3,#4)#5{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
\addto@pscode{%
    \variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
	/Hpyramide #5 def
    tx@3DDict begin
	SommetsPyramide
	PSDA 0 le { %
	    reduction reduction scale
	    newpath
	    1 setlinejoin
	    /Xabscisse XS 1 fracHeight sub XD XS sub mul add def
	    /Yordonnee YS 1 fracHeight sub YD YS sub mul add def
		/Zcote ZS CZ sub fracHeight mul CZ add def
	    CalcCoordinates
		moveto
	    /Xabscisse XD def
	    /Yordonnee YD def
	    /Zcote ZD def
	    CalcCoordinates
	    lineto
	    /Xabscisse XA def
	    /Yordonnee YA def
	    /Zcote ZA def
	    CalcCoordinates
	    lineto
	    /Xabscisse XS 1 fracHeight sub XA XS sub mul add def
	    /Yordonnee YS 1 fracHeight sub YA YS sub mul add def
		/Zcote ZS CZ sub fracHeight mul CZ add def
	    CalcCoordinates
		lineto
	    closepath
	} if
    end
}% fin du code ps
\end@ClosedObj
}}
%
\def\FaceABCD{\pst@object{FaceABCD}}
\def\FaceABCD@i{\@ifnextchar[{\FaceABCD@do}{\FaceABCD@do[]}}
\def\FaceABCD@do[#1](#2,#3,#4)#5{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
    \addto@pscode{%
	\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
	/Hpyramide #5 def
	tx@3DDict begin
	SommetsPyramide
	PSABCD 0 le { %
	    reduction reduction scale
	    newpath
	    1 setlinejoin
	    /Xabscisse XA def
	    /Yordonnee YA def
	    /Zcote ZA def
	    CalcCoordinates
    	    moveto
	    /Xabscisse XB def
	    /Yordonnee YB def
	    /Zcote ZB def
	    CalcCoordinates
	    lineto
	    /Xabscisse XC def
	    /Yordonnee YC def
	    /Zcote ZC def
	    CalcCoordinates
	    lineto
	    /Xabscisse XD def
	    /Yordonnee YD def
	    /Zcote ZD def
	    CalcCoordinates
	    lineto
	    closepath
	} if
	end
    }% fin du code ps
\end@ClosedObj
}}
%
% hv 2003
\def\FaceABCDTop{\pst@object{FaceABCDTop}}
\def\FaceABCDTop@i{\@ifnextchar[{\FaceABCDTop@do}{\FaceABCDTop@do[]}}
\def\FaceABCDTop@do[#1](#2,#3,#4)#5{{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
    \addto@pscode{%
	\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
	/Hpyramide #5 def
	tx@3DDict begin
	SommetsPyramide
	PSABCD 0 gt { %
	    reduction reduction scale
	    newpath
	    1 setlinejoin
	    /Xabscisse XS 1 fracHeight sub XD XS sub mul add def
	    /Yordonnee YS 1 fracHeight sub YD YS sub mul add def
	    /Zcote ZS CZ sub fracHeight mul CZ add def
	    CalcCoordinates
   	    moveto
	    /Xabscisse XS 1 fracHeight sub XA XS sub mul add def
	    /Yordonnee YS 1 fracHeight sub YA YS sub mul add def
	    /Zcote ZS CZ sub fracHeight mul CZ add def
	    CalcCoordinates
	    lineto
	    /Xabscisse XS 1 fracHeight sub XB XS sub mul add def
	    /Yordonnee YS 1 fracHeight sub YB YS sub mul add def
	    /Zcote ZS CZ sub fracHeight mul CZ add def
	    CalcCoordinates
	    lineto
	    /Xabscisse XS 1 fracHeight sub XC XS sub mul add def
	    /Yordonnee YS 1 fracHeight sub YC YS sub mul add def
	    /Zcote ZS CZ sub fracHeight mul CZ add def
	    CalcCoordinates
	    lineto
	    closepath
	} if
	end
    }% fin du code ps
\end@ClosedObj
}}
%
\def\PyramideThreeD{\@ifnextchar[{\@PyramideThreeD}{\@PyramideThreeD[]}}
% (#2,#3,#4) the coordinates of the origin
% #5 the height of the pyrimide
\def\@PyramideThreeD[#1](#2,#3,#4)#5{{%
%    \setkeys{psset}{#1}%
%	\setkeys{psset}{CX=#2,CY=#3,CZ=#4,Hpyramide=#5}% makes the values globally
%    \pst@object{PyramideThreeD}%
%}}
%\def\PyramideThreeD@i{%
    \FaceSAB[fillcolor=\psk@TroisD@TetraedreColorFaceA][#1](#2,#3,#4){#5}%
    \FaceSBC[fillcolor=\psk@TroisD@TetraedreColorFaceB][#1](#2,#3,#4){#5}%
    \FaceSCD[fillcolor=\psk@TroisD@TetraedreColorFaceC][#1](#2,#3,#4){#5}%
    \FaceSDA[fillcolor=\psk@TroisD@TetraedreColorFaceD][#1](#2,#3,#4){#5}%
    \FaceABCD[fillcolor=\psk@TroisD@TetraedreColorFaceE][#1](#2,#3,#4){#5}%
%    \ifnum\psk@TroisD@fracHeight < 1
	\FaceABCDTop[fillcolor=\psk@TroisD@TetraedreColorFaceE][#1](#2,#3,#4){#5}%
%    \fi
}}
%
%
\def\ConeThreeD{\pst@object{ConeThreeD}}
\def\ConeThreeD@i{\@ifnextchar[{\ConeThreeD@do}{\ConeThreeD@do[]}}
\def\ConeThreeD@do[#1](#2,#3,#4)#5#6{{%
% Le centre de la base sera placé avec
% (#2,#3,#4) les paramètres CX,CY et CZ
% #5 rayon
% #6 hauteur
% on peut ensuite faire tourner le cylindre
% avec RotX, RotY et RotZ
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
	\addto@pscode{%
		\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
		reduction reduction scale
    	/Rcone #5 def
    	/Hcone #6 def
		tx@3DDict begin
			ConeThreeD
		end
	}% fin du code ps
	\showpointsfalse
\end@ClosedObj
}}%
%
\def\CircleThreeD{\pst@object{CircleThreeD}}
\def\CircleThreeD@i{\@ifnextchar[{\CircleThreeD@do}{\CircleThreeD@do[]}}
\def\CircleThreeD@do[#1](#2,#3,#4)#5{{%
% (#2,#3,#4) les paramètres CX,CY et CZ
% #5 rayon du cercle
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
    \addto@pscode{%
	/Rcercle #5 def
	\variablesTroisD
	\ifPst@SphericalCoor
		/Radius #2 def
		/longitude #3 def
		/latitude #4 def
		/CZ Radius latitude sin mul def
		/CX Radius longitude cos mul latitude cos mul def
		/CY Radius longitude sin mul latitude cos mul def
	\else
		/CX #2 def
		/CY #3 def
		/CZ #4 def
	\fi
	tx@3DDict begin
    	    reduction reduction scale
	    /TableauxPoints [
	    0 1 359 {% on décrit le cercle
		/Angle exch def [
		    /Xcercle Rcercle Angle cos mul def
		    /Ycercle Rcercle Angle sin mul def
		    /Xabscisse Xcercle S1 mul Ycercle S2 C1 mul mul add CX add def
		    /Yordonnee Xcercle C1 mul neg Ycercle S2 S1 mul mul add CY add def
		    /Zcote Ycercle C2 mul neg CZ add def
		    CalcCoordinates ]
	    } for
	    ] def
	    TableauxPoints 0 get aload pop moveto
	    0 1 359 {
		/compteur exch def
		TableauxPoints compteur get aload pop
	    lineto } for
	end
	}% fin du code ps
	\showpointsfalse
\end@ClosedObj
}}
%
%
\def\FrameThreeD{\pst@object{FrameThreeD}}
\def\FrameThreeD@i{\@ifnextchar[{\FrameThreeD@do}{\FrameThreeD@do[]}}
\def\FrameThreeD@do[#1](#2,#3,#4)(#5,#6)(#7,#8){{%
% (#2,#3,#4) the origin
% (#5,#6) d'un sommet
% (#7,#8) du sommet opposé
% rectangle ABCD
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
	\addto@pscode{%
		/XA #5 def
		/YA #6 def
		/XC #7 def
		/YC #8 def
% on en déduit les autres sommets
		/XB XC def
		/YB YA def
		/XD XA def
		/YD YC def
		\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
		tx@3DDict begin
			reduction reduction scale
			newpath
		    /Xframe XA def
			/Yframe YA def
		    /Xabscisse Xframe S1 mul Yframe S2 C1 mul mul add CX add def
		    /Yordonnee Xframe C1 mul neg Yframe S2 S1 mul mul add CY add def
		    /Zcote Yframe C2 mul neg CZ add def
		    CalcCoordinates
		     moveto
		    /Xframe XB def
		    /Yframe YB def
		    /Xabscisse Xframe S1 mul Yframe S2 C1 mul mul add CX add def
		    /Yordonnee Xframe C1 mul neg Yframe S2 S1 mul mul add CY add def
		    /Zcote Yframe C2 mul neg CZ add def
		    CalcCoordinates
		    lineto
		    /Xframe XC def
		    /Yframe YC def
		    /Xabscisse Xframe S1 mul Yframe S2 C1 mul mul add CX add def
		    /Yordonnee Xframe C1 mul neg Yframe S2 S1 mul mul add CY add def
		    /Zcote Yframe C2 mul neg CZ add def
		    CalcCoordinates
		    lineto
		    /Xframe XD def
		    /Yframe YD def
		    /Xabscisse Xframe S1 mul Yframe S2 C1 mul mul add CX add def
		    /Yordonnee Xframe C1 mul neg Yframe S2 S1 mul mul add CY add def
		    /Zcote Yframe C2 mul neg CZ add def
		    CalcCoordinates
		    lineto
		    /Xframe XA def
		    /Yframe YA def
		    /Xabscisse Xframe S1 mul Yframe S2 C1 mul mul add CX add def
		    /Yordonnee Xframe C1 mul neg Yframe S2 S1 mul mul add CY add def
		    /Zcote Yframe C2 mul neg CZ add def
		    CalcCoordinates
		    lineto
			closepath
		end
	}% fin du code ps
	\showpointsfalse
\end@ClosedObj
}}% % fin de la commande PSTricks
%
%
\def\QuadrillageThreeD{\pst@object{QuadrillageThreeD}}
\def\QuadrillageThreeD@i{\@ifnextchar[{\QuadrillageThreeD@do}{\QuadrillageThreeD@do[]}}
\def\QuadrillageThreeD@do[#1](#2,#3,#4)(#5,#6)(#7,#8){{%
\pst@killglue
\setkeys{psset}{#1}%
\begin@OpenObj
	\addto@pscode{%
		\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
		/Xmin #5 def
		/Xmax #7 def
		/Ymin #6 def
		/Ymax #8 def
		/pas \psk@TroisD@pas\space def
		/grille \psk@TroisD@grille\space def
		tx@3DDict begin
			reduction reduction scale
			Ymin grille Ymax {% balayage suivant Oy
			/Ygrille exch def
			/TableauxPoints [
			Xmin pas Xmax { % balayage suivant Ox
				/Xgrille exch def
				/Xabscisse Xgrille S1 mul Ygrille S2 C1 mul mul add CX add def
				/Yordonnee Xgrille C1 mul neg Ygrille S2 S1 mul mul add CY add def
				/Zcote Ygrille C2 mul neg CZ add def
				formulesTroisD
				[ Xi 28.45 mul Yi 28.45 mul ]
			} for
    		] def
			TableauxPoints 0 get aload pop moveto
			0 1 Xmax Xmin sub pas div {
				/compteur exch def
				TableauxPoints compteur get aload pop
				lineto
			} for
% stroke
    		} for
%
			Xmin grille Xmax {% balayage suivant Ox
    		/Xgrille exch def
			/TableauxPoints [
				Ymin pas Ymax { % balayage suivant Ox
				/Ygrille exch def
				/Xabscisse Xgrille S1 mul Ygrille S2 C1 mul mul add CX add def
				/Yordonnee Xgrille C1 mul neg Ygrille S2 S1 mul mul add CY add def
				/Zcote Ygrille C2 mul neg CZ add def
				formulesTroisD
				[ Xi 28.45 mul Yi 28.45 mul ]
        		} for
    		] def
			TableauxPoints 0 get aload pop moveto
			0 1 Ymax Ymin sub pas div {
				/compteur exch def
    			TableauxPoints compteur get aload pop
   				lineto
			} for
			\pst@number\pslinewidth SLW
  			\pst@usecolor\pslinecolor
			\@nameuse{psls@\pslinestyle}
% stroke
    		} for
% fin du tracé
		end
	}% fin du code ps
\end@OpenObj
}}% % fin de la commande PSTricks
%
%
% 11 novembre
\def\DemiSphereThreeD{\pst@object{DemiSphereThreeD}}
\def\DemiSphereThreeD@i{\@ifnextchar[{\DemiSphereThreeD@do}{\DemiSphereThreeD@do[]}}
\def\DemiSphereThreeD@do[#1](#2,#3,#4)#5{{%
% (#2,#3,#4) coordinates of the center
% #5 rayon
	\pst@killglue
	\setkeys{psset}{#1}%
	\begin@ClosedObj
		\addto@pscode{%
			\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
			reduction reduction scale
    		/Rsphere #5 def
    		/increment 10 def
			tx@3DDict begin
				/condition {PSfacette 0 le} def
				/departPhi 0 def
				MaillageSphere
% centre de la base inférieure après transformations
			    /CxFaceInf CX def
			    /CyFaceInf CY def
			    /CzFaceInf CZ def
% correction 16 novembre 2002
%    /Xpoint CxFaceInf def
%    /Ypoint CyFaceInf def
%    /Zpoint CzFaceInf def
			    /Xpoint 0 def
			    /Ypoint 0 def
			    /Zpoint 0 def
% fin correction 16/11/2002
				CalculsPointsAfterTransformations
 			   /CxBaseInf Xabscisse def
		    /CyBaseInf Yordonnee def
    /CzBaseInf Zcote def
    /RXvueInf CxBaseInf XpointVue sub def
    /RYvueInf CyBaseInf YpointVue sub def
    /RZvueInf CzBaseInf ZpointVue sub def
% Sommet de la sphère
    /Xpoint 0 def
    /Ypoint 0 def
    /Zpoint Rsphere def
CalculsPointsAfterTransformations
    /XsommetSphere Xabscisse def
    /YsommetSphere Yordonnee def
    /ZsommetSphere Zcote def
% Normale extérieure à la base inférieure
    /nXBaseInf CxFaceInf XsommetSphere sub def
    /nYBaseInf CyFaceInf YsommetSphere sub def
    /nZBaseInf CzFaceInf ZsommetSphere sub def
% Visibilité de la base inférieure
    /PSbaseSphere nXBaseInf RXvueInf mul
                  nYBaseInf RYvueInf mul add
                  nZBaseInf RZvueInf mul add def
PSbaseSphere 0 le {
/TableauxPoints [
0 1 359 {% on décrit le cercle
    /theta exch def [
    /Xpoint Rsphere theta cos mul def
    /Ypoint Rsphere theta sin mul def
    /Zpoint 0 def
CalculsPointsAfterTransformations
    CalcCoordinates ]
    } for
    ] def
gsave
newpath
 TableauxPoints 0 get aload pop moveto
0 1 359 {
    /compteur exch def
    TableauxPoints compteur get aload pop
    lineto } for
0.7 setgray
closepath
fill
grestore
 } if
end
 }% fin du code ps
\showpointsfalse
\end@ClosedObj
 }}% % fin de la commande PSTricks
%
%
\def\SphereCreuseThreeD{\pst@object{SphereCreuseThreeD}}
\def\SphereCreuseThreeD@i{\@ifnextchar[{\SphereCreuseThreeD@do}{\SphereCreuseThreeD@do[]}}
\def\SphereCreuseThreeD@do[#1](#2,#3,#4)#5{{%
% (#2,#3,#4) coordinates of the center
% #5 rayon
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
	\addto@pscode{%
		\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
		reduction reduction scale
		/Rsphere #5 def
		/increment 10 def
		tx@3DDict begin
			/SphereInside {
				/condition {PSfacette 0 ge} def
				/departPhi 0 def
				MaillageSphere
			} def
%
% centre de la base inférieure après transformations
			/CxFaceInf CX def
			/CyFaceInf CY def
			/CzFaceInf CZ def
			/Xpoint CxFaceInf def
			/Ypoint CyFaceInf def
			/Zpoint CzFaceInf def
			CalculsPointsAfterTransformations
			/CxBaseInf Xabscisse def
			/CyBaseInf Yordonnee def
			/CzBaseInf Zcote def
			/RXvueInf CxBaseInf XpointVue sub def
			/RYvueInf CyBaseInf YpointVue sub def
			/RZvueInf CzBaseInf ZpointVue sub def
% Sommet de la sphère
			/Xpoint 0 def
			/Ypoint 0 def
			/Zpoint Rsphere def
			CalculsPointsAfterTransformations
			/XsommetSphere Xabscisse def
			/YsommetSphere Yordonnee def
			/ZsommetSphere Zcote def
% Normale extérieure à la base inférieure
			/nXBaseInf CxFaceInf XsommetSphere sub def
			/nYBaseInf CyFaceInf YsommetSphere sub def
			/nZBaseInf CzFaceInf ZsommetSphere sub def
% Visibilité de la base inférieure
			/PSbaseSphere nXBaseInf RXvueInf mul nYBaseInf RYvueInf mul add
				nZBaseInf RZvueInf mul add def
			/base {
				/TableauxPoints [
					0 1 359 {% on décrit le cercle
						/theta exch def [
						/Xpoint Rsphere theta cos mul def
						/Ypoint Rsphere theta sin mul def
						/Zpoint 0 def
						CalculsPointsAfterTransformations
						CalcCoordinates ]
					} for
				] def
% gsave
				newpath
				TableauxPoints 0 get aload pop moveto
				0 1 359 {
					/compteur exch def
					TableauxPoints compteur get aload pop
				lineto } for
				0.7 setgray
				closepath
				% stroke
				%grestore
			} def
			PSbaseSphere 0 le {
				base
				clip
				SphereInside
			}{ 0 0 0.01 0 360 arc } ifelse
		end
	}% fin du code ps
	\showpointsfalse
	\end@ClosedObj
}}% % fin de la commande PSTricks
%
% 30 novembre 2002
% révisé le 30 octobre 2003
\def\PortionSphereThreeD{\pst@object{PortionSphereThreeD}}
\def\PortionSphereThreeD@i{\@ifnextchar[{\PortionSphereThreeD@do}{\PortionSphereThreeD@do[]}}
\def\PortionSphereThreeD@do[#1](#2,#3,#4)#5{{%
% (#2,#3,#4) coordinates of the center
% #5 rayon
\pst@killglue
\setkeys{psset}{#1}%
\begin@ClosedObj
	\addto@pscode{%
		\variablesTroisD
		\ifPst@SphericalCoor
			/Radius #2 def
			/longitude #3 def
			/latitude #4 def
			/CZ Radius latitude sin mul def
			/CX Radius longitude cos mul latitude cos mul def
			/CY Radius longitude sin mul latitude cos mul def
		\else
			/CX #2 def
			/CY #3 def
			/CZ #4 def
		\fi
		reduction reduction scale
    	/Rsphere #5 def
    	/increment 1 def
%    	/increment 2.5 def
		tx@3DDict begin
  			PortionSphere
		end
 	}% fin du code ps
	\showpointsfalse
\end@ClosedObj
}}% % fin de la commande PSTricks
%
%% END: pst-vue3D.tex
\endinput

%% ChangeLog
% 1.0g	2003-12-21	hv: fixed a bug in \pNodeThreeD
% 1.0f	2003-12-20	hv: added two eye macros, drop the options for
%                       CX,CY,CZ and Xorigine,...
%                       added option SphericalCoor and modify all
%                       macros to use it
% 1.0e	2003-12-18	hv: edit the \AxesThreeD macro
% 1.0d	2003-12-18	hv: fix bug in truncated pyramid

